FairMedFM: Fairness Benchmarking for Medical Imaging Foundation Models

The advent of foundation models (FMs) in healthcare offers unprecedented opportunities to enhance medical diagnostics through automated classification and segmentation tasks. However, these models also raise significant concerns about their fairness, especially when applied to diverse and underrepresented populations in healthcare applications. Currently, there is a lack of comprehensive benchmarks, standardized pipelines, and easily adaptable libraries to evaluate and understand the fairness performance of FMs in medical imaging, leading to considerable challenges in formulating and implementing solutions that ensure equitable outcomes across diverse patient populations. To fill this gap, we introduce FairMedFM, a fairness benchmark for FM research in medical imaging.FairMedFM integrates with 17 popular medical imaging datasets, encompassing different modalities, dimensionalities, and sensitive attributes. It explores 20 widely used FMs, with various usages such as zero-shot learning, linear probing, parameter-efficient fine-tuning, and prompting in various downstream tasks -- classification and segmentation. Our exhaustive analysis evaluates the fairness performance over different evaluation metrics from multiple perspectives, revealing the existence of bias, varied utility-fairness trade-offs on different FMs, consistent disparities on the same datasets regardless FMs, and limited effectiveness of existing unfairness mitigation methods. Checkout FairMedFM's project page and open-sourced codebase, which supports extendible functionalities and applications as well as inclusive for studies on FMs in medical imaging over the long term.

==> sections/full_res_cls.tex <==
% \begin{table}[htbp]

% \centering
% \caption{Classification results for ADNI, BREST, CheXpert, and COVID dataset, \textit{sex} as the sensitive attribute. All experiments are repeated three times and $\text{mean}\pm\text{std}$ are reported (\%).}    
% % \adjustbox{width = \textwidth, height=}{
% \resizebox*{0.6\textheight}{!}{
% \begin{threeparttable}
% \begin{tabular}{cccrrrrrrrrrrrrrr}
% \toprule
% \textbf{Dataset} & \textbf{Usage} & \textbf{Model}&\textbf{AUC}&\textbf{ACC}&\textbf{BCE}&\textbf{ECE}&$\Delta$\textbf{AUC}&$\Delta$\textbf{ECE}&\textbf{DP}&\textbf{EOD}&\textbf{AUC}$_{\text{Male}}$&\textbf{AUC}$_{\text{Female}}$&\textbf{ECE}$_{\text{Male}}$&\textbf{ECE}$_{\text{Female}}$ \\
% \midrule
% \multirow{23}{*}{{\rotatebox{90}{ADNI}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP &55.79$\pm$2.52&47.76$\pm$0.45&69.32$\pm$0.29&16.27$\pm$2.38&16.44$\pm$8.24&4.87$\pm$2.75&5.77$\pm$3.33&12.01$\pm$2.38&53.12$\pm$4.22&56.73$\pm$11.93&16.21$\pm$4.14&14.90$\pm$7.57 \\
% & & BLIP2 &56.75$\pm$4.53&49.04$\pm$6.23&68.29$\pm$1.20&13.15$\pm$1.68&14.95$\pm$4.61&3.68$\pm$2.72&10.90$\pm$6.18&9.91$\pm$7.26&59.06$\pm$6.35&57.76$\pm$2.03&14.37$\pm$3.07&13.60$\pm$1.86 \\
% & & BioMedCLIP &56.54$\pm$2.27&48.40$\pm$6.58&69.89$\pm$1.02&14.08$\pm$2.56&10.29$\pm$7.16&3.09$\pm$1.23&9.62$\pm$5.77&10.11$\pm$2.34&64.93$\pm$3.84&55.50$\pm$10.68&21.10$\pm$5.31&25.37$\pm$5.68 \\
% & & C2L &56.13$\pm$7.35&46.79$\pm$9.10&69.50$\pm$0.41&14.50$\pm$2.51&6.86$\pm$6.81&3.51$\pm$1.84&2.56$\pm$1.11&3.99$\pm$3.22&63.39$\pm$2.77&66.26$\pm$3.15&15.16$\pm$3.46&18.63$\pm$1.98 \\
% & & CLIP &55.49$\pm$0.68&41.03$\pm$0.45&69.22$\pm$0.15&14.34$\pm$3.93&1.84$\pm$1.04&4.50$\pm$3.34&2.56$\pm$1.11&5.33$\pm$7.30&57.86$\pm$4.22&55.91$\pm$1.87&14.88$\pm$5.34&12.98$\pm$5.14 \\
% & & DINOv2 &57.87$\pm$4.22&54.17$\pm$5.05&67.97$\pm$0.66&12.79$\pm$1.23&9.58$\pm$3.69&4.21$\pm$5.16&1.92$\pm$0.00&8.53$\pm$1.18&71.02$\pm$2.31&77.01$\pm$1.98&19.57$\pm$2.20&15.23$\pm$3.28 \\
% & & MedCLIP &57.17$\pm$3.70&45.83$\pm$4.32&69.37$\pm$0.22&14.54$\pm$1.47&6.45$\pm$4.41&2.50$\pm$0.88&3.21$\pm$2.94&4.53$\pm$0.00&66.21$\pm$0.00&52.84$\pm$0.00&17.53$\pm$0.00&25.69$\pm$0.00 \\
% & & MedLVM &55.98$\pm$7.33&42.31$\pm$2.36&68.64$\pm$1.45&14.46$\pm$1.48&11.16$\pm$9.59&3.73$\pm$2.03&5.13$\pm$7.28&6.40$\pm$0.00&58.37$\pm$0.00&54.69$\pm$0.00&26.91$\pm$0.00&27.59$\pm$0.00 \\
% & & MedMAE &56.95$\pm$5.16&48.40$\pm$6.68&69.06$\pm$0.25&11.67$\pm$0.39&6.30$\pm$4.64&5.63$\pm$1.62&8.33$\pm$1.11&7.50$\pm$0.93&56.53$\pm$1.08&44.70$\pm$1.87&58.69$\pm$1.17&58.65$\pm$1.32 \\
% & & MoCo-CXR &47.60$\pm$10.58&45.51$\pm$7.94&69.85$\pm$0.96&14.66$\pm$1.57&4.58$\pm$2.74&3.25$\pm$0.44&10.26$\pm$16.13&11.73$\pm$0.00&41.32$\pm$0.00&70.66$\pm$0.00&22.50$\pm$0.00&10.99$\pm$0.00 \\
% & & PubMedCLIP &59.30$\pm$5.26&55.45$\pm$8.65&69.17$\pm$0.03&15.30$\pm$2.10&8.06$\pm$7.60&2.64$\pm$2.85&8.33$\pm$11.10&10.93$\pm$2.31&53.51$\pm$2.94&56.84$\pm$11.96&23.48$\pm$2.63&24.74$\pm$0.75 \\
% \cline{2-15}
% & \multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP &59.41$\pm$0.00&64.42$\pm$0.00&68.88$\pm$0.00&16.23$\pm$0.00&13.36$\pm$0.00&8.17$\pm$0.00&13.46$\pm$0.00&15.13$\pm$0.00&31.09$\pm$0.00&66.41$\pm$0.00&29.08$\pm$0.00&33.16$\pm$0.00 \\
% & & BLIP2 &56.41$\pm$0.00&42.31$\pm$0.00&80.20$\pm$0.00&25.47$\pm$0.00&3.69$\pm$0.00&0.68$\pm$0.00&3.85$\pm$0.00&3.99$\pm$4.18&56.02$\pm$14.95&48.70$\pm$11.96&22.47$\pm$0.75&27.42$\pm$2.73 \\
% & & BioMedCLIP &51.30$\pm$0.78&39.74$\pm$0.56&338.74$\pm$50.21&58.58$\pm$1.41&11.83$\pm$2.94&0.10$\pm$0.10&1.28$\pm$1.11&2.92$\pm$0.00&84.03$\pm$0.00&75.78$\pm$0.00&27.13$\pm$0.00&30.30$\pm$0.00 \\
% & & CLIP &55.61$\pm$0.00&39.42$\pm$0.00&70.44$\pm$0.00&14.81$\pm$0.00&29.34$\pm$0.00&11.51$\pm$0.00&1.92$\pm$0.00&2.38$\pm$2.67&45.69$\pm$19.99&54.43$\pm$15.06&26.93$\pm$5.46&19.53$\pm$2.59\\
% & & MedCLIP &55.25$\pm$7.56&49.68$\pm$6.75&75.45$\pm$2.56&22.72$\pm$1.59&8.04$\pm$1.55&2.19$\pm$1.25&4.49$\pm$2.22&6.94$\pm$13.25&65.50$\pm$6.61&62.00$\pm$6.61&25.55$\pm$3.63&20.79$\pm$2.84\\
% & & PubMedCLIP &53.03$\pm$0.00&41.35$\pm$0.00&75.07$\pm$0.00&18.19$\pm$0.00&25.35$\pm$0.00&0.50$\pm$0.00&5.77$\pm$0.00&5.61$\pm$11.31&56.99$\pm$9.52&67.13$\pm$5.72&20.38$\pm$2.13&29.01$\pm$2.68\\
% \cline{2-15}
% & \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP &54.71$\pm$5.30&47.76$\pm$4.74&69.65$\pm$2.16&12.47$\pm$2.32&12.42$\pm$1.65&8.29$\pm$2.23&1.92$\pm$1.92&6.37$\pm$0.05&77.25$\pm$0.00&76.34$\pm$0.00&35.49$\pm$0.00&32.84$\pm$0.00\\
% & & BLIP2 &58.60$\pm$3.11&49.36$\pm$8.40&67.54$\pm$0.63&13.22$\pm$4.13&4.84$\pm$3.82&1.48$\pm$1.67&10.26$\pm$10.59&13.31$\pm$0.02&83.22$\pm$0.00&83.78$\pm$0.01&26.79$\pm$0.01&27.52$\pm$0.01\\
% & & BioMedCLIP &60.55$\pm$6.02&57.05$\pm$8.18&76.88$\pm$5.66&17.39$\pm$1.38&9.42$\pm$8.54&6.97$\pm$7.77&10.26$\pm$1.11&11.98$\pm$0.04&89.21$\pm$0.00&90.32$\pm$0.00&21.78$\pm$0.10&22.01$\pm$0.09\\
% & & CLIP &65.40$\pm$2.70&57.05$\pm$6.26&65.49$\pm$1.16&10.48$\pm$2.37&2.87$\pm$2.30&5.19$\pm$2.26&1.28$\pm$1.11&2.92$\pm$0.06&82.78$\pm$0.01&83.54$\pm$0.01&28.44$\pm$0.00&27.63$\pm$0.02\\
% & & MedCLIP &57.33$\pm$1.68&50.32$\pm$2.42&67.41$\pm$0.20&10.18$\pm$3.65&4.30$\pm$0.86&3.36$\pm$3.12&8.33$\pm$9.87&9.34$\pm$0.07&83.87$\pm$0.00&84.96$\pm$0.00&28.67$\pm$0.00&28.67$\pm$0.01\\
% & & PubMedCLIP &74.45$\pm$0.56&69.23$\pm$2.54&62.60$\pm$0.33&13.22$\pm$2.57&5.99$\pm$4.02&4.34$\pm$4.76&17.95$\pm$1.11&17.36$\pm$1.89&81.85$\pm$0.28&82.53$\pm$0.20&32.28$\pm$0.26&29.64$\pm$0.07\\
% \midrule
% \multirow{23}{*}{{\rotatebox{90}{BREST}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP &84.21$\pm$0.11&92.15$\pm$0.57&50.84$\pm$0.09&32.02$\pm$0.07&6.15$\pm$0.10&3.99$\pm$0.05&0.62$\pm$0.24&9.43$\pm$0.00&40.09$\pm$0.00&65.44$\pm$0.00&19.18$\pm$0.00&19.68$\pm$0.00 \\
% & & BLIP2 &91.61$\pm$0.08&94.64$\pm$0.13&38.09$\pm$0.04&23.89$\pm$0.04&0.27$\pm$0.06&3.02$\pm$0.04&1.06$\pm$0.19&7.35$\pm$4.39&50.03$\pm$7.07&60.78$\pm$10.49&18.28$\pm$3.28&16.90$\pm$2.26\\
% & & BioMedCLIP &85.09$\pm$0.19&92.42$\pm$0.46&43.81$\pm$0.03&25.87$\pm$0.07&7.06$\pm$0.28&2.86$\pm$0.16&0.23$\pm$0.18&4.59$\pm$5.18&60.34$\pm$13.18&53.69$\pm$3.94&17.99$\pm$1.38&14.32$\pm$2.57\\
% & & C2L &77.32$\pm$0.17&85.27$\pm$1.09&65.76$\pm$0.32&40.94$\pm$0.19&6.16$\pm$0.29&2.74$\pm$0.02&3.13$\pm$0.57&12.10$\pm$7.16&58.55$\pm$8.96&55.79$\pm$5.83&16.22$\pm$0.95&17.13$\pm$2.20\\
% & & CLIP &84.76$\pm$0.12&91.00$\pm$0.41&53.53$\pm$0.06&34.06$\pm$0.03&6.83$\pm$0.15&3.12$\pm$0.14&0.69$\pm$0.08&9.19$\pm$2.79&57.53$\pm$4.84&54.61$\pm$12.15&18.31$\pm$1.62&18.42$\pm$2.60\\
% & & DINOv2 &91.35$\pm$0.11&94.95$\pm$0.22&33.05$\pm$0.07&19.55$\pm$0.06&3.67$\pm$0.08&2.70$\pm$0.10&0.54$\pm$0.13&5.60$\pm$1.22&54.99$\pm$1.28&56.27$\pm$0.96&14.09$\pm$2.25&18.59$\pm$4.95\\
% & & MedCLIP &78.05$\pm$0.18&83.18$\pm$4.10&50.51$\pm$0.24&30.41$\pm$0.17&4.17$\pm$0.40&1.96$\pm$0.01&1.80$\pm$0.96&1.88$\pm$4.41&58.58$\pm$9.02&55.97$\pm$2.85&16.82$\pm$4.53&19.32$\pm$0.94\\
% & & MedLVM &85.56$\pm$0.09&91.50$\pm$0.00&49.16$\pm$0.13&30.01$\pm$0.10&3.09$\pm$0.05&1.69$\pm$0.01&1.54$\pm$0.42&4.74$\pm$1.64&60.37$\pm$1.00&53.92$\pm$5.13&19.39$\pm$3.11&18.10$\pm$0.98\\
% & & MedMAE &70.58$\pm$0.20&71.08$\pm$2.86&64.09$\pm$0.04&39.45$\pm$0.02&0.17$\pm$0.15&1.34$\pm$0.04&3.38$\pm$0.59&3.76$\pm$5.62&55.53$\pm$14.18&56.71$\pm$7.80&17.92$\pm$0.82&15.32$\pm$3.93\\
% & & MoCo-CXR &82.17$\pm$1.22&91.52$\pm$0.54&56.54$\pm$0.74&35.49$\pm$0.57&3.18$\pm$1.10&2.52$\pm$0.16&0.81$\pm$0.25&2.14$\pm$0.49&55.48$\pm$4.50&61.11$\pm$6.71&17.11$\pm$4.95&17.99$\pm$2.09\\
% & & PubMedCLIP &80.64$\pm$0.02&90.08$\pm$1.02&56.35$\pm$0.06&35.45$\pm$0.04&12.15$\pm$0.09&2.19$\pm$0.04&0.71$\pm$0.53&9.67$\pm$14.81&47.11$\pm$11.19&47.08$\pm$10.37&19.23$\pm$2.88&20.02$\pm$0.34\\
% \cline{2-15}
% & \multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP &40.59$\pm$0.00&7.52$\pm$0.00&453.89$\pm$0.00&91.42$\pm$0.00&1.38$\pm$0.00&2.61$\pm$0.00&0.12$\pm$0.00&0.98$\pm$2.02&55.83$\pm$7.13&61.89$\pm$10.58&29.32$\pm$0.15&24.99$\pm$8.86\\
% & & BLIP2 &50.00$\pm$0.05&61.45$\pm$27.39&335.77$\pm$0.00&89.86$\pm$0.00&1.05$\pm$0.12&2.51$\pm$0.00&0.54$\pm$0.25&0.86$\pm$7.25&61.89$\pm$12.71&38.46$\pm$6.07&22.78$\pm$4.32&22.33$\pm$2.58\\
% & & BioMedCLIP &78.16$\pm$0.46&85.27$\pm$0.56&28.62$\pm$0.86&5.58$\pm$1.50&2.95$\pm$0.91&2.74$\pm$2.24&3.84$\pm$1.39&11.38$\pm$3.59&55.24$\pm$9.09&39.74$\pm$7.39&22.34$\pm$10.64&27.45$\pm$0.43\\
% & & CLIP &61.23$\pm$0.00&76.96$\pm$0.00&88.43$\pm$0.00&52.17$\pm$0.00&2.85$\pm$0.00&1.74$\pm$0.00&3.08$\pm$0.00&4.50$\pm$2.72&40.33$\pm$14.41&48.25$\pm$2.80&24.45$\pm$7.26&23.01$\pm$6.28\\
% & & MedCLIP &52.18$\pm$7.78&54.80$\pm$40.43&67.79$\pm$4.02&41.58$\pm$2.25&6.64$\pm$6.07&2.63$\pm$0.05&1.54$\pm$1.18&3.47$\pm$2.45&42.77$\pm$9.84&45.57$\pm$1.58&27.74$\pm$4.74&25.29$\pm$5.53\\
% & & PubMedCLIP &50.33$\pm$0.00&63.28$\pm$0.00&192.25$\pm$0.00&79.51$\pm$0.00&9.73$\pm$0.00&2.38$\pm$0.00&4.16$\pm$0.00&10.73$\pm$0.00&41.96$\pm$4.59&53.38$\pm$5.05&25.41$\pm$3.66&21.27$\pm$3.58\\
% \cline{2-15}
% & \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP &89.39$\pm$0.02&94.48$\pm$0.07&16.59$\pm$0.01&1.81$\pm$0.06&3.02$\pm$0.04&1.38$\pm$0.03&1.96$\pm$0.14&3.30$\pm$0.14&78.81$\pm$0.00&78.43$\pm$0.00&33.55$\pm$0.00&31.22$\pm$0.00\\
% & & BLIP2 &85.01$\pm$0.03&91.87$\pm$0.21&20.58$\pm$0.02&3.10$\pm$0.00&2.76$\pm$0.08&0.25$\pm$0.21&1.35$\pm$0.13&0.53$\pm$0.36&77.29$\pm$0.02&73.48$\pm$0.01&3.64$\pm$0.21&3.41$\pm$0.05 \\
% & & BioMedCLIP &88.08$\pm$0.09&94.60$\pm$0.40&16.58$\pm$0.05&0.70$\pm$0.14&1.20$\pm$0.18&0.64$\pm$0.26&1.85$\pm$0.24&2.49$\pm$0.49&74.81$\pm$0.33&71.67$\pm$0.12&4.66$\pm$0.16&4.88$\pm$1.15 \\
% & & CLIP &87.76$\pm$0.00&92.57$\pm$0.07&18.51$\pm$0.00&1.65$\pm$0.03&1.74$\pm$0.00&0.26$\pm$0.01&2.29$\pm$0.00&1.00$\pm$0.17&74.11$\pm$0.04&71.06$\pm$0.16&4.51$\pm$0.29&3.78$\pm$0.35 \\
% & & MedCLIP &89.29$\pm$0.51&94.11$\pm$0.62&17.97$\pm$0.13&3.36$\pm$0.08&2.78$\pm$0.08&0.60$\pm$0.38&1.89$\pm$0.24&1.96$\pm$0.18&75.32$\pm$0.05&73.41$\pm$0.00&4.28$\pm$0.12&2.88$\pm$0.24 \\
% & & PubMedCLIP &83.44$\pm$0.00&93.10$\pm$0.00&19.98$\pm$0.00&1.99$\pm$0.02&2.69$\pm$0.03&0.58$\pm$0.02&1.25$\pm$0.00&3.43$\pm$0.16&77.02$\pm$0.33&73.51$\pm$0.47&4.24$\pm$0.77&3.52$\pm$0.59 \\
% \midrule
% \multirow{23}{*}{{\rotatebox{90}{CheXpert}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP &77.90$\pm$0.00&81.69$\pm$0.02&56.10$\pm$0.00&31.22$\pm$0.00&0.76$\pm$0.00&2.33$\pm$0.00&3.27$\pm$0.03&5.28$\pm$4.17&53.89$\pm$6.58&49.97$\pm$11.28&40.26$\pm$2.24&42.89$\pm$2.24 \\
% & & BLIP2 &82.91$\pm$0.00&84.55$\pm$0.04&51.63$\pm$0.00&28.48$\pm$0.00&0.07$\pm$0.00&0.50$\pm$0.00&1.20$\pm$0.01&2.50$\pm$0.00&54.15$\pm$0.00&44.42$\pm$0.00&78.39$\pm$0.00&80.77$\pm$0.00 \\
% & & BioMedCLIP &83.60$\pm$0.00&84.81$\pm$0.02&50.30$\pm$0.00&26.29$\pm$0.00&0.77$\pm$0.00&1.59$\pm$0.01&1.72$\pm$0.02&2.16$\pm$2.03&82.07$\pm$0.14&88.22$\pm$0.07&30.04$\pm$0.08&34.03$\pm$0.08\\
% & & C2L &81.88$\pm$0.00&84.94$\pm$0.00&65.53$\pm$0.00&38.26$\pm$0.00&1.45$\pm$0.00&0.11$\pm$0.00&0.04$\pm$0.00&2.00$\pm$0.85&91.81$\pm$0.10&91.53$\pm$0.09&22.36$\pm$0.05&25.38$\pm$0.03\\
% & & CLIP &76.61$\pm$0.00&81.01$\pm$0.00&59.32$\pm$0.00&34.16$\pm$0.00&0.91$\pm$0.00&2.65$\pm$0.00&2.71$\pm$0.02&4.83$\pm$0.27&82.21$\pm$0.07&89.26$\pm$0.34&24.42$\pm$0.05&27.28$\pm$0.12\\
% & & DINOv2 &83.49$\pm$0.00&85.54$\pm$0.02&50.12$\pm$0.01&27.16$\pm$0.01&0.55$\pm$0.01&0.73$\pm$0.01&0.77$\pm$0.02&1.16$\pm$2.35&75.09$\pm$0.31&81.26$\pm$0.16&39.56$\pm$0.20&42.30$\pm$0.18\\
% & & MedCLIP &89.77$\pm$0.00&89.33$\pm$0.02&43.04$\pm$0.14&21.90$\pm$0.09&1.11$\pm$0.00&0.23$\pm$0.01&1.04$\pm$0.01&2.77$\pm$0.74&82.03$\pm$0.16&88.85$\pm$0.11&32.68$\pm$0.05&35.80$\pm$0.16\\
% & & MedLVM &83.15$\pm$0.01&86.44$\pm$0.01&51.27$\pm$0.02&28.03$\pm$0.01&0.76$\pm$0.00&0.81$\pm$0.02&1.21$\pm$0.03&1.40$\pm$1.36&89.92$\pm$0.08&93.59$\pm$0.15&18.18$\pm$0.10&20.88$\pm$0.03\\
% & & MedMAE &84.39$\pm$0.00&86.30$\pm$0.45&51.14$\pm$0.01&28.67$\pm$0.01&1.08$\pm$0.00&0.00$\pm$0.00&1.63$\pm$0.01&2.05$\pm$1.10&76.26$\pm$0.36&80.42$\pm$0.11&29.41$\pm$0.17&31.38$\pm$0.17\\
% & & MoCo-CXR &82.04$\pm$0.22&84.61$\pm$0.52&54.27$\pm$0.19&30.96$\pm$0.16&0.69$\pm$0.09&2.64$\pm$0.26&5.40$\pm$1.24&7.81$\pm$2.47&84.26$\pm$0.10&87.34$\pm$0.07&29.16$\pm$0.10&30.84$\pm$0.10\\
% & & PubMedCLIP &78.51$\pm$0.00&83.92$\pm$0.17&56.81$\pm$0.00&32.38$\pm$0.00&0.38$\pm$0.00&2.33$\pm$0.00&2.13$\pm$0.03&3.77$\pm$2.98&70.37$\pm$0.13&70.53$\pm$0.28&38.78$\pm$0.01&40.12$\pm$0.04\\
% \cline{2-15}
% & \multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP &56.08$\pm$0.00&38.14$\pm$0.00&79.90$\pm$0.00&45.73$\pm$0.00&2.44$\pm$0.00&0.62$\pm$0.00&5.89$\pm$0.00&3.62$\pm$0.10&81.21$\pm$0.18&81.78$\pm$0.07&0.63$\pm$0.10&0.91$\pm$0.10 \\
% & & BLIP2 &63.65$\pm$0.00&64.14$\pm$1.41&49.85$\pm$0.00&25.71$\pm$0.00&3.57$\pm$0.01&0.27$\pm$0.00&9.11$\pm$0.08&11.81$\pm$0.04&82.12$\pm$0.00&82.66$\pm$0.00&0.70$\pm$0.01&0.91$\pm$0.01 \\
% & & BioMedCLIP &72.50$\pm$2.33&81.90$\pm$2.47&155.70$\pm$8.82&48.73$\pm$3.22&2.62$\pm$0.52&4.87$\pm$1.17&2.26$\pm$1.20&2.81$\pm$0.00&57.33$\pm$0.00&54.89$\pm$0.00&45.42$\pm$0.00&46.04$\pm$0.00 \\
% & & CLIP &54.05$\pm$0.00&29.15$\pm$0.00&120.38$\pm$0.00&61.80$\pm$0.00&1.61$\pm$0.00&0.66$\pm$0.00&2.97$\pm$0.00&3.26$\pm$0.35&61.87$\pm$0.00&65.44$\pm$0.01&25.58$\pm$0.00&25.85$\pm$0.00 \\
% & & MedCLIP &48.27$\pm$14.32&30.77$\pm$35.66&72.37$\pm$7.10&41.48$\pm$4.02&3.71$\pm$1.01&1.09$\pm$0.29&4.25$\pm$7.29&5.32$\pm$1.58&71.20$\pm$2.46&73.82$\pm$2.24&46.32$\pm$3.77&51.18$\pm$2.61 \\
% & & PubMedCLIP &67.45$\pm$0.00&76.79$\pm$0.00&66.14$\pm$0.00&38.26$\pm$0.00&0.81$\pm$0.00&0.57$\pm$0.00&3.78$\pm$0.00&4.15$\pm$0.00&53.18$\pm$0.00&54.79$\pm$0.00&61.47$\pm$0.00&62.13$\pm$0.00 \\
% \cline{2-15}
% & \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP &79.94$\pm$0.00&85.22$\pm$0.03&27.04$\pm$0.00&0.75$\pm$0.01&0.36$\pm$0.00&0.05$\pm$0.00&0.37$\pm$0.01&0.75$\pm$0.00&49.81$\pm$0.00&50.30$\pm$0.00&13.84$\pm$0.00&15.04$\pm$0.00 \\
% & & BLIP2 &81.65$\pm$0.74&85.32$\pm$0.51&26.43$\pm$0.43&1.14$\pm$0.46&0.55$\pm$0.26&0.25$\pm$0.12&0.33$\pm$0.12&0.46$\pm$0.99&72.82$\pm$0.05&67.05$\pm$0.03&6.61$\pm$0.30&2.33$\pm$0.05\\
% & & BioMedCLIP &84.07$\pm$0.00&86.06$\pm$0.31&25.20$\pm$0.00&0.68$\pm$0.01&0.88$\pm$0.00&0.37$\pm$0.07&1.51$\pm$0.09&2.00$\pm$0.78&75.78$\pm$0.01&72.52$\pm$0.03&5.65$\pm$0.07&3.30$\pm$0.10\\
% & & CLIP &81.23$\pm$0.00&84.83$\pm$0.03&26.52$\pm$0.00&0.76$\pm$0.01&0.16$\pm$0.00&0.14$\pm$0.01&0.87$\pm$0.04&2.00$\pm$0.52&73.86$\pm$0.08&68.83$\pm$0.02&2.76$\pm$0.32&4.69$\pm$0.31\\
% & & MedCLIP &81.50$\pm$0.10&85.35$\pm$0.64&26.39$\pm$0.05&0.69$\pm$0.06&0.56$\pm$0.18&0.27$\pm$0.01&0.20$\pm$0.08&0.56$\pm$0.11&71.24$\pm$0.02&68.09$\pm$0.01&12.10$\pm$0.15&10.14$\pm$0.10\\
% & & PubMedCLIP &82.37$\pm$0.00&85.27$\pm$0.01&25.92$\pm$0.00&0.55$\pm$0.01&0.54$\pm$0.00&0.21$\pm$0.01&1.50$\pm$0.01&2.53$\pm$0.64&70.51$\pm$0.07&66.25$\pm$0.06&7.09$\pm$0.48&5.44$\pm$0.47\\
% \midrule
% \multirow{23}{*}{{\rotatebox{90}{COVID}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP &50.67$\pm$13.90&54.17$\pm$7.41&69.35$\pm$0.63&17.05$\pm$1.71&15.73$\pm$12.24&7.40$\pm$5.34&2.78$\pm$2.41&6.76$\pm$9.29&55.07$\pm$8.75&63.13$\pm$1.41&19.17$\pm$2.71&16.60$\pm$1.72\\
% & & BLIP2 &59.84$\pm$5.78&59.03$\pm$7.67&69.12$\pm$0.36&18.11$\pm$3.34&9.56$\pm$6.31&7.46$\pm$3.27&20.83$\pm$15.02&20.40$\pm$0.42&88.31$\pm$0.02&91.33$\pm$0.02&1.76$\pm$0.02&3.14$\pm$0.01 \\
% & & BioMedCLIP &60.47$\pm$3.71&60.42$\pm$2.95&69.28$\pm$1.42&18.82$\pm$3.35&10.14$\pm$11.34&8.63$\pm$5.70&15.28$\pm$16.84&18.53$\pm$0.37&83.94$\pm$0.05&86.70$\pm$0.03&2.50$\pm$0.03&2.75$\pm$0.23 \\
% & & C2L &57.03$\pm$1.56&51.39$\pm$1.96&69.26$\pm$0.02&15.66$\pm$4.73&12.82$\pm$10.23&9.56$\pm$2.52&8.33$\pm$0.00&9.56$\pm$0.26&87.62$\pm$0.16&88.83$\pm$0.03&1.80$\pm$0.20&1.17$\pm$0.08 \\
% & & CLIP &50.58$\pm$4.06&52.78$\pm$4.28&69.45$\pm$0.22&13.84$\pm$2.42&23.43$\pm$18.65&4.52$\pm$3.45&11.11$\pm$6.36&11.66$\pm$0.14&88.64$\pm$0.00&86.89$\pm$0.00&2.27$\pm$0.02&2.01$\pm$0.03 \\
% & & DINOv2 &50.38$\pm$2.22&53.47$\pm$3.93&74.38$\pm$6.31&19.57$\pm$4.32&17.83$\pm$12.45&10.77$\pm$5.50&6.94$\pm$4.81&7.58$\pm$1.09&88.21$\pm$0.49&91.00$\pm$0.52&2.97$\pm$0.22&3.57$\pm$0.29 \\
% & & MedCLIP &45.46$\pm$6.96&49.31$\pm$0.98&69.70$\pm$0.44&18.87$\pm$2.11&9.79$\pm$9.25&11.90$\pm$8.11&6.94$\pm$2.41&7.58$\pm$0.00&82.38$\pm$0.01&85.08$\pm$0.01&2.12$\pm$0.02&2.70$\pm$0.01 \\
% & & MedLVM &43.72$\pm$5.38&52.08$\pm$1.70&70.81$\pm$0.48&21.29$\pm$6.72&7.93$\pm$2.46&5.59$\pm$1.92&6.94$\pm$2.41&7.34$\pm$0.00&41.43$\pm$0.00&40.05$\pm$0.00&90.10$\pm$0.00&92.71$\pm$0.00 \\
% & & MedMAE &45.57$\pm$1.58&47.92$\pm$0.00&70.17$\pm$0.56&16.68$\pm$1.77&11.42$\pm$9.45&7.23$\pm$2.28&4.17$\pm$0.00&3.85$\pm$0.38&49.53$\pm$0.00&50.58$\pm$0.12&88.58$\pm$0.00&91.10$\pm$0.00 \\
% & & MoCo-CXR &45.31$\pm$10.21&52.08$\pm$2.95&69.62$\pm$0.27&17.81$\pm$3.50&12.94$\pm$11.04&6.35$\pm$6.44&9.72$\pm$6.36&11.31$\pm$3.15&77.42$\pm$0.45&80.37$\pm$0.89&5.98$\pm$1.42&6.20$\pm$2.83 \\
% & & PubMedCLIP &47.74$\pm$7.21&47.92$\pm$1.70&69.42$\pm$0.09&19.02$\pm$1.59&3.73$\pm$3.85&2.73$\pm$2.27&6.94$\pm$2.41&7.34$\pm$0.00&59.93$\pm$0.00&62.78$\pm$0.00&51.29$\pm$0.00&53.03$\pm$0.00 \\
% \cline{2-15}
% & \multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP &56.36$\pm$0.00&66.67$\pm$0.00&88.44$\pm$0.00&26.92$\pm$0.00&33.21$\pm$0.00&7.53$\pm$0.00&4.17$\pm$0.00&2.94$\pm$6.54&38.34$\pm$13.47&51.28$\pm$8.11&18.55$\pm$2.40&21.22$\pm$6.15\\
% & & BLIP2 &63.43$\pm$0.00&75.00$\pm$0.00&78.25$\pm$0.00&23.95$\pm$0.00&11.04$\pm$0.00&8.25$\pm$0.00&12.50$\pm$0.00&19.54$\pm$2.45&48.60$\pm$8.22&44.87$\pm$7.19&22.71$\pm$4.00&19.98$\pm$2.18\\
% & & BioMedCLIP &91.78$\pm$1.54&84.03$\pm$2.41&57.67$\pm$6.37&21.46$\pm$1.75&5.42$\pm$0.82&1.98$\pm$0.93&5.56$\pm$4.81&5.48$\pm$0.01&79.77$\pm$0.00&80.12$\pm$0.00&0.78$\pm$0.00&0.83$\pm$0.00 \\
% & & CLIP &50.51$\pm$0.00&66.67$\pm$0.00&192.06$\pm$0.00&31.06$\pm$0.00&35.31$\pm$0.00&4.07$\pm$0.00&4.17$\pm$0.00&3.12$\pm$0.20&81.37$\pm$0.61&81.92$\pm$0.87&1.21$\pm$0.53&1.24$\pm$0.22 \\
% & & MedCLIP &51.18$\pm$7.29&68.06$\pm$1.20&66.94$\pm$2.50&17.24$\pm$3.96&15.61$\pm$3.91&4.96$\pm$2.19&6.94$\pm$2.41&7.70$\pm$0.07&83.65$\pm$0.00&84.53$\pm$0.00&0.53$\pm$0.03&0.91$\pm$0.04 \\
% & & PubMedCLIP &81.21$\pm$0.00&77.08$\pm$0.00&76.95$\pm$0.00&26.57$\pm$0.00&8.25$\pm$0.00&3.17$\pm$0.00&16.67$\pm$0.00&14.84$\pm$0.04&81.17$\pm$0.00&81.32$\pm$0.00&0.85$\pm$0.00&0.72$\pm$0.01 \\
% \cline{2-15}
% & \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP &65.25$\pm$10.53&71.53$\pm$5.24&64.80$\pm$8.86&15.86$\pm$2.31&9.03$\pm$6.54&7.38$\pm$0.18&8.33$\pm$4.17&8.72$\pm$0.17&75.60$\pm$0.01&71.66$\pm$0.01&3.36$\pm$0.02&4.83$\pm$0.11 \\
% & & BLIP2 &66.60$\pm$15.35&69.44$\pm$3.18&62.49$\pm$3.90&17.69$\pm$1.77&12.41$\pm$8.95&2.60$\pm$2.05&6.94$\pm$2.41&8.30$\pm$0.00&42.18$\pm$0.00&46.67$\pm$0.00&21.20$\pm$0.00&18.06$\pm$0.00 \\
% & & BioMedCLIP &94.61$\pm$1.35&88.19$\pm$1.20&25.18$\pm$3.28&6.43$\pm$0.24&2.53$\pm$0.41&4.10$\pm$1.88&8.33$\pm$4.17&7.83$\pm$0.00&42.47$\pm$0.01&45.42$\pm$0.01&18.23$\pm$0.00&18.84$\pm$0.04 \\
% & & CLIP &64.51$\pm$14.24&68.75$\pm$3.61&65.51$\pm$8.40&21.79$\pm$4.29&11.79$\pm$9.19&5.69$\pm$0.61&5.56$\pm$2.41&6.09$\pm$0.00&53.24$\pm$2.94&55.37$\pm$1.89&30.59$\pm$10.08&28.52$\pm$8.93 \\
% & & MedCLIP &64.38$\pm$18.56&73.61$\pm$6.70&61.69$\pm$4.93&18.52$\pm$3.10&12.30$\pm$3.22&5.03$\pm$4.51&6.94$\pm$2.41&8.10$\pm$0.00&60.04$\pm$0.00&60.33$\pm$0.00&15.03$\pm$0.00&15.43$\pm$0.00 \\
% & & PubMedCLIP &87.00$\pm$2.37&78.47$\pm$2.41&47.34$\pm$1.97&15.74$\pm$3.49&3.07$\pm$1.16&4.45$\pm$3.79&25.00$\pm$0.00&28.01$\pm$0.11&54.30$\pm$7.19&54.20$\pm$5.65&7.39$\pm$3.30&7.10$\pm$2.69 \\
% \bottomrule
% \end{tabular}
% \end{threeparttable}
% }
% % \end{sidewaystable}
% \end{table}

\begin{table}[htbp]

\centering
\caption{Classification results for ADNI, BREST, and COVID datasets, \textit{sex} as the sensitive attribute. All experiments are repeated three times and $\text{mean}\pm\text{std}$ are reported (\%).}    
\label{tab:full_res_cls_1}
% \adjustbox{width = \textwidth, height=}{
\resizebox*{0.6\textheight}{!}{
\begin{threeparttable}
\begin{tabular}{cccrrrrrrrrrrrrrr}
\toprule
\textbf{Dataset} & \textbf{Usage} & \textbf{Model}&\textbf{AUC}&\textbf{ACC}&\textbf{BCE}&\textbf{ECE}&$\Delta$\textbf{AUC}&$\Delta$\textbf{ECE}&\textbf{DP}&\textbf{EOD}&\textbf{AUC}$_{\text{Male}}$&\textbf{AUC}$_{\text{Female}}$&\textbf{ECE}$_{\text{Male}}$&\textbf{ECE}$_{\text{Female}}$ \\
\midrule
\multirow{23}{*}{{\rotatebox{90}{ADNI}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP & 55.79$\pm$2.52 & 47.76$\pm$0.45 & 69.32$\pm$0.29 & 16.27$\pm$2.38 & 16.44$\pm$8.24 & 4.87$\pm$2.75 & 5.77$\pm$3.33 & 12.01$\pm$4.39 & 50.03$\pm$7.07 & 60.78$\pm$10.49 & 18.28$\pm$3.28 & 16.90$\pm$2.26\\
& & BLIP2 & 56.75$\pm$4.53 & 49.04$\pm$6.23 & 68.29$\pm$1.20 & 13.15$\pm$1.68 & 14.95$\pm$4.61 & 3.68$\pm$2.72 & 10.90$\pm$6.18 & 9.91$\pm$5.18 & 60.34$\pm$13.18 & 53.69$\pm$3.94 & 17.99$\pm$1.38 & 14.32$\pm$2.57\\
& & BiomedCLIP & 56.54$\pm$2.27 & 48.40$\pm$6.58 & 69.89$\pm$1.02 & 14.08$\pm$2.56 & 10.29$\pm$7.16 & 3.09$\pm$1.23 & 9.62$\pm$5.77 & 10.11$\pm$7.16 & 58.55$\pm$8.96 & 55.79$\pm$5.83 & 16.22$\pm$0.95 & 17.13$\pm$2.20\\
& & C2L & 56.13$\pm$7.35 & 46.79$\pm$9.10 & 69.50$\pm$0.41 & 14.50$\pm$2.51 & 6.86$\pm$6.81 & 3.51$\pm$1.84 & 2.56$\pm$1.11 & 3.99$\pm$2.79 & 57.53$\pm$4.84 & 54.61$\pm$12.15 & 18.31$\pm$1.62 & 18.42$\pm$2.60\\
& & CLIP & 55.49$\pm$0.68 & 41.03$\pm$0.45 & 69.22$\pm$0.15 & 14.34$\pm$3.93 & 1.84$\pm$1.04 & 4.50$\pm$3.34 & 2.56$\pm$1.11 & 5.33$\pm$1.22 & 54.99$\pm$1.28 & 56.27$\pm$0.96 & 14.09$\pm$2.25 & 18.59$\pm$4.95\\
& & DINOv2 & 57.87$\pm$4.22 & 54.17$\pm$5.05 & 67.97$\pm$0.66 & 12.79$\pm$1.23 & 9.58$\pm$3.69 & 4.21$\pm$5.16 & 1.92$\pm$0.00 & 8.53$\pm$4.41 & 58.58$\pm$9.02 & 55.97$\pm$2.85 & 16.82$\pm$4.53 & 19.32$\pm$0.94\\
& & MedCLIP & 57.17$\pm$3.70 & 45.83$\pm$4.32 & 69.37$\pm$0.22 & 14.54$\pm$1.47 & 6.45$\pm$4.41 & 2.50$\pm$0.88 & 3.21$\pm$2.94 & 4.53$\pm$1.64 & 60.37$\pm$1.00 & 53.92$\pm$5.13 & 19.39$\pm$3.11 & 18.10$\pm$0.98\\
& & MedLVM & 55.98$\pm$7.33 & 42.31$\pm$2.36 & 68.64$\pm$1.45 & 14.46$\pm$1.48 & 11.16$\pm$9.59 & 3.73$\pm$2.03 & 5.13$\pm$7.28 & 6.40$\pm$5.62 & 55.53$\pm$14.18 & 56.71$\pm$7.80 & 17.92$\pm$0.82 & 15.32$\pm$3.93\\
& & MedMAE & 56.95$\pm$5.16 & 48.40$\pm$6.68 & 69.06$\pm$0.25 & 11.67$\pm$0.39 & 6.30$\pm$4.64 & 5.63$\pm$1.62 & 8.33$\pm$1.11 & 7.50$\pm$0.49 & 55.48$\pm$4.50 & 61.11$\pm$6.71 & 17.11$\pm$4.95 & 17.99$\pm$2.09\\
&& MoCo-CXR & 47.60$\pm$10.58 & 45.51$\pm$7.94 & 69.85$\pm$0.96 & 14.66$\pm$1.57 & 4.58$\pm$2.74 & 3.25$\pm$0.44 & 10.26$\pm$16.13 & 11.73$\pm$14.81 & 47.11$\pm$11.19 & 47.08$\pm$10.37 & 19.23$\pm$2.88 & 20.02$\pm$0.34\\
& & PubMedCLIP & 59.30$\pm$5.26 & 55.45$\pm$8.65 & 69.17$\pm$0.03 & 15.30$\pm$2.10 & 8.06$\pm$7.60 & 2.64$\pm$2.85 & 8.33$\pm$11.10 & 10.93$\pm$9.29 & 55.07$\pm$8.75 & 63.13$\pm$1.41 & 19.17$\pm$2.71 & 16.60$\pm$1.72\\
\cline{2-15}
 & \multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP & 59.41$\pm$0.00 & 64.42$\pm$0.00 & 68.88$\pm$0.00 & 16.23$\pm$0.00 & 13.36$\pm$0.00 & 8.17$\pm$0.00 & 13.46$\pm$0.00 & 84.87$\pm$0.00 & 66.21$\pm$0.00 & 52.84$\pm$0.00 & 17.53$\pm$0.00 & 25.69$\pm$0.00\\
 & & BLIP2 & 56.41$\pm$0.00 & 42.31$\pm$0.00 & 80.20$\pm$0.00 & 25.47$\pm$0.00 & 3.69$\pm$0.00 & 0.68$\pm$0.00 & 3.85$\pm$0.00 & 96.01$\pm$0.00 & 58.37$\pm$0.00 & 54.69$\pm$0.00 & 26.91$\pm$0.00 & 27.59$\pm$0.00\\
 & & BiomedCLIP & 51.30$\pm$0.78 & 39.74$\pm$0.56 & 338.74$\pm$50.21 & 58.58$\pm$1.41 & 11.83$\pm$2.94 & 0.10$\pm$0.10 & 1.28$\pm$1.11 & 97.08$\pm$0.93 & 56.53$\pm$1.08 & 44.70$\pm$1.87 & 58.69$\pm$1.17 & 58.65$\pm$1.32\\
&  & CLIP & 55.61$\pm$0.00 & 39.42$\pm$0.00 & 70.44$\pm$0.00 & 14.81$\pm$0.00 & 29.34$\pm$0.00 & 11.51$\pm$0.00 & 1.92$\pm$0.00 & 97.62$\pm$0.00 & 41.32$\pm$0.00 & 70.66$\pm$0.00 & 22.50$\pm$0.00 & 10.99$\pm$0.00\\
 &  & MedCLIP & 55.25$\pm$7.56 & 49.68$\pm$6.75 & 75.45$\pm$2.56 & 22.72$\pm$1.59 & 8.04$\pm$1.55 & 2.19$\pm$1.25 & 4.49$\pm$2.22 & 93.06$\pm$2.31 & 53.51$\pm$2.94 & 56.84$\pm$11.96 & 23.48$\pm$2.63 & 24.74$\pm$0.75\\
 &  & PubMedCLIP & 53.03$\pm$0.00 & 41.35$\pm$0.00 & 75.07$\pm$0.00 & 18.19$\pm$0.00 & 25.35$\pm$0.00 & 0.50$\pm$0.00 & 5.77$\pm$0.00 & 94.39$\pm$0.00 & 40.09$\pm$0.00 & 65.44$\pm$0.00 & 19.18$\pm$0.00 & 19.68$\pm$0.00\\
\cline{2-15}
 &  \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP & 54.71$\pm$5.30 & 47.76$\pm$4.74 & 69.65$\pm$2.16 & 12.47$\pm$2.32 & 12.42$\pm$1.65 & 8.29$\pm$2.23 & 1.92$\pm$1.92 & 93.63$\pm$2.38 & 53.12$\pm$4.22 & 56.73$\pm$11.93 & 16.21$\pm$4.14 & 14.90$\pm$7.57\\
 & & BLIP2 & 58.60$\pm$3.11 & 49.36$\pm$8.40 & 67.54$\pm$0.63 & 13.22$\pm$4.13 & 4.84$\pm$3.82 & 1.48$\pm$1.67 & 10.26$\pm$10.59 & 86.69$\pm$7.26 & 59.06$\pm$6.35 & 57.76$\pm$2.03 & 14.37$\pm$3.07 & 13.60$\pm$1.86\\
 & & BiomedCLIP & 60.55$\pm$6.02 & 57.05$\pm$8.18 & 76.88$\pm$5.66 & 17.39$\pm$1.38 & 9.42$\pm$8.54 & 6.97$\pm$7.77 & 10.26$\pm$1.11 & 88.02$\pm$2.34 & 64.93$\pm$3.84 & 55.50$\pm$10.68 & 21.10$\pm$5.31 & 25.37$\pm$5.68\\
 & & CLIP & 65.40$\pm$2.70 & 57.05$\pm$6.26 & 65.49$\pm$1.16 & 10.48$\pm$2.37 & 2.87$\pm$2.30 & 5.19$\pm$2.26 & 1.28$\pm$1.11 & 97.08$\pm$3.22 & 63.39$\pm$2.77 & 66.26$\pm$3.15 & 15.16$\pm$3.46 & 18.63$\pm$1.98\\
&  & MedCLIP & 57.33$\pm$1.68 & 50.32$\pm$2.42 & 67.41$\pm$0.20 & 10.18$\pm$3.65 & 4.30$\pm$0.86 & 3.36$\pm$3.12 & 8.33$\pm$9.87 & 90.66$\pm$7.30 & 57.86$\pm$4.22 & 55.91$\pm$1.87 & 14.88$\pm$5.34 & 12.98$\pm$5.14\\
&  & PubMedCLIP & 74.45$\pm$0.56 & 69.23$\pm$2.54 & 62.60$\pm$0.33 & 13.22$\pm$2.57 & 5.99$\pm$4.02 & 4.34$\pm$4.76 & 17.95$\pm$1.11 & 82.64$\pm$1.18 & 71.02$\pm$2.31 & 77.01$\pm$1.98 & 19.57$\pm$2.20 & 15.23$\pm$3.28\\
\midrule
\multirow{23}{*}{{\rotatebox{90}{BERST}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP & 84.21$\pm$0.11 & 92.15$\pm$0.57 & 50.84$\pm$0.09 & 32.02$\pm$0.07 & 6.15$\pm$0.10 & 3.99$\pm$0.05 & 0.62$\pm$0.24 & 9.43$\pm$2.03 & 82.07$\pm$0.14 & 88.22$\pm$0.07 & 30.04$\pm$0.08 & 34.03$\pm$0.08\\
& & BLIP2 & 91.61$\pm$0.08 & 94.64$\pm$0.13 & 38.09$\pm$0.04 & 23.89$\pm$0.04 & 0.27$\pm$0.06 & 3.02$\pm$0.04 & 1.06$\pm$0.19 & 7.35$\pm$0.85 & 91.81$\pm$0.10 & 91.53$\pm$0.09 & 22.36$\pm$0.05 & 25.38$\pm$0.03\\
& & BiomedCLIP & 85.09$\pm$0.19 & 92.42$\pm$0.46 & 43.81$\pm$0.03 & 25.87$\pm$0.07 & 7.06$\pm$0.28 & 2.86$\pm$0.16 & 0.23$\pm$0.18 & 4.59$\pm$0.27 & 82.21$\pm$0.07 & 89.26$\pm$0.34 & 24.42$\pm$0.05 & 27.28$\pm$0.12\\
& & C2L & 77.32$\pm$0.17 & 85.27$\pm$1.09 & 65.76$\pm$0.32 & 40.94$\pm$0.19 & 6.16$\pm$0.29 & 2.74$\pm$0.02 & 3.13$\pm$0.57 & 12.10$\pm$2.35 & 75.09$\pm$0.31 & 81.26$\pm$0.16 & 39.56$\pm$0.20 & 42.30$\pm$0.18\\
& & CLIP & 84.76$\pm$0.12 & 91.00$\pm$0.41 & 53.53$\pm$0.06 & 34.06$\pm$0.03 & 6.83$\pm$0.15 & 3.12$\pm$0.14 & 0.69$\pm$0.08 & 9.19$\pm$0.74 & 82.03$\pm$0.16 & 88.85$\pm$0.11 & 32.68$\pm$0.05 & 35.80$\pm$0.16\\
& & DINOv2 & 91.35$\pm$0.11 & 94.95$\pm$0.22 & 33.05$\pm$0.07 & 19.55$\pm$0.06 & 3.67$\pm$0.08 & 2.70$\pm$0.10 & 0.54$\pm$0.13 & 5.60$\pm$1.36 & 89.92$\pm$0.08 & 93.59$\pm$0.15 & 18.18$\pm$0.10 & 20.88$\pm$0.03\\
& & MedCLIP & 78.05$\pm$0.18 & 83.18$\pm$4.10 & 50.51$\pm$0.24 & 30.41$\pm$0.17 & 4.17$\pm$0.40 & 1.96$\pm$0.01 & 1.80$\pm$0.96 & 1.88$\pm$1.10 & 76.26$\pm$0.36 & 80.42$\pm$0.11 & 29.41$\pm$0.17 & 31.38$\pm$0.17\\
& & MedLVM & 85.56$\pm$0.09 & 91.50$\pm$0.00 & 49.16$\pm$0.13 & 30.01$\pm$0.10 & 3.09$\pm$0.05 & 1.69$\pm$0.01 & 1.54$\pm$0.42 & 4.74$\pm$2.47 & 84.26$\pm$0.10 & 87.34$\pm$0.07 & 29.16$\pm$0.10 & 30.84$\pm$0.10\\
& & MedMAE & 70.58$\pm$0.20 & 71.08$\pm$2.86 & 64.09$\pm$0.04 & 39.45$\pm$0.02 & 0.17$\pm$0.15 & 1.34$\pm$0.04 & 3.38$\pm$0.59 & 3.76$\pm$2.98 & 70.37$\pm$0.13 & 70.53$\pm$0.28 & 38.78$\pm$0.01 & 40.12$\pm$0.04\\
& & MoCo-CXR & 82.17$\pm$1.22 & 91.52$\pm$0.54 & 56.54$\pm$0.74 & 35.49$\pm$0.57 & 3.18$\pm$1.10 & 2.52$\pm$0.16 & 0.81$\pm$0.25 & 2.14$\pm$2.13 & 80.85$\pm$1.34 & 84.03$\pm$1.26 & 34.22$\pm$0.51 & 36.74$\pm$0.62\\
& & PubMedCLIP & 80.64$\pm$0.02 & 90.08$\pm$1.02 & 56.35$\pm$0.06 & 35.45$\pm$0.04 & 12.15$\pm$0.09 & 2.19$\pm$0.04 & 0.71$\pm$0.53 & 9.67$\pm$0.72 & 75.38$\pm$0.06 & 87.53$\pm$0.04 & 34.42$\pm$0.04 & 36.61$\pm$0.05\\
\cline{2-15}
  & \multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP & 40.59$\pm$0.00 & 7.52$\pm$0.00 & 453.89$\pm$0.00 & 91.42$\pm$0.00 & 1.38$\pm$0.00 & 2.61$\pm$0.00 & 0.12$\pm$0.00 & 99.02$\pm$0.00 & 41.43$\pm$0.00 & 40.05$\pm$0.00 & 90.10$\pm$0.00 & 92.71$\pm$0.00\\
& & BLIP2 & 50.00$\pm$0.05 & 61.45$\pm$27.39 & 335.77$\pm$0.00 & 89.86$\pm$0.00 & 1.05$\pm$0.12 & 2.51$\pm$0.00 & 0.54$\pm$0.25 & 99.14$\pm$0.38 & 49.53$\pm$0.00 & 50.58$\pm$0.12 & 88.58$\pm$0.00 & 91.10$\pm$0.00\\
& & BiomedCLIP & 78.16$\pm$0.46 & 85.27$\pm$0.56 & 28.62$\pm$0.86 & 5.58$\pm$1.50 & 2.95$\pm$0.91 & 2.74$\pm$2.24 & 3.84$\pm$1.39 & 88.62$\pm$3.15 & 77.42$\pm$0.45 & 80.37$\pm$0.89 & 5.98$\pm$1.42 & 6.20$\pm$2.83\\
& & CLIP & 61.23$\pm$0.00 & 76.96$\pm$0.00 & 88.43$\pm$0.00 & 52.17$\pm$0.00 & 2.85$\pm$0.00 & 1.74$\pm$0.00 & 3.08$\pm$0.00 & 95.50$\pm$0.00 & 59.93$\pm$0.00 & 62.78$\pm$0.00 & 51.29$\pm$0.00 & 53.03$\pm$0.00\\
& & MedCLIP & 52.18$\pm$7.78 & 54.80$\pm$40.43 & 67.79$\pm$4.02 & 41.58$\pm$2.25 & 6.64$\pm$6.07 & 2.63$\pm$0.05 & 1.54$\pm$1.18 & 96.53$\pm$4.17 & 53.89$\pm$6.58 & 49.97$\pm$11.28 & 40.26$\pm$2.24 & 42.89$\pm$2.24\\
&& PubMedCLIP & 50.33$\pm$0.00 & 63.28$\pm$0.00 & 192.25$\pm$0.00 & 79.51$\pm$0.00 & 9.73$\pm$0.00 & 2.38$\pm$0.00 & 4.16$\pm$0.00 & 89.27$\pm$0.00 & 54.15$\pm$0.00 & 44.42$\pm$0.00 & 78.39$\pm$0.00 & 80.77$\pm$0.00\\
\cline{2-15}
  & \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP & 89.39$\pm$0.02 & 94.48$\pm$0.07 & 16.59$\pm$0.01 & 1.81$\pm$0.06 & 3.02$\pm$0.04 & 1.38$\pm$0.03 & 1.96$\pm$0.14 & 96.70$\pm$0.42 & 88.31$\pm$0.02 & 91.33$\pm$0.02 & 1.76$\pm$0.02 & 3.14$\pm$0.01\\
& & BLIP2 & 85.01$\pm$0.03 & 91.87$\pm$0.21 & 20.58$\pm$0.02 & 3.10$\pm$0.00 & 2.76$\pm$0.08 & 0.25$\pm$0.21 & 1.35$\pm$0.13 & 99.47$\pm$0.37 & 83.94$\pm$0.05 & 86.70$\pm$0.03 & 2.50$\pm$0.03 & 2.75$\pm$0.23\\
&& BiomedCLIP & 88.08$\pm$0.09 & 94.60$\pm$0.40 & 16.58$\pm$0.05 & 0.70$\pm$0.14 & 1.20$\pm$0.18 & 0.64$\pm$0.26 & 1.85$\pm$0.24 & 97.51$\pm$0.26 & 87.62$\pm$0.16 & 88.83$\pm$0.03 & 1.80$\pm$0.20 & 1.17$\pm$0.08\\
& & CLIP & 87.76$\pm$0.00 & 92.57$\pm$0.07 & 18.51$\pm$0.00 & 1.65$\pm$0.03 & 1.74$\pm$0.00 & 0.26$\pm$0.01 & 2.29$\pm$0.00 & 99.00$\pm$0.14 & 88.64$\pm$0.00 & 86.89$\pm$0.00 & 2.27$\pm$0.02 & 2.01$\pm$0.03\\
& & MedCLIP & 89.29$\pm$0.51 & 94.11$\pm$0.62 & 17.97$\pm$0.13 & 3.36$\pm$0.08 & 2.78$\pm$0.08 & 0.60$\pm$0.38 & 1.89$\pm$0.24 & 98.04$\pm$1.09 & 88.21$\pm$0.49 & 91.00$\pm$0.52 & 2.97$\pm$0.22 & 3.57$\pm$0.29\\
& & PubMedCLIP & 83.44$\pm$0.00 & 93.10$\pm$0.00 & 19.98$\pm$0.00 & 1.99$\pm$0.02 & 2.69$\pm$0.03 & 0.58$\pm$0.02 & 1.25$\pm$0.00 & 96.57$\pm$0.00 & 82.38$\pm$0.01 & 85.08$\pm$0.01 & 2.12$\pm$0.02 & 2.70$\pm$0.01\\

\midrule
\multirow{23}{*}{{\rotatebox{90}{COVID}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP & 50.67$\pm$13.90 & 54.17$\pm$7.41 & 69.35$\pm$0.63 & 17.05$\pm$1.71 & 15.73$\pm$12.24 & 7.40$\pm$5.34 & 2.78$\pm$2.41 & 6.76$\pm$2.67 & 45.69$\pm$19.99 & 54.43$\pm$15.06 & 26.93$\pm$5.46 & 19.53$\pm$2.59\\
&  & BLIP2 & 59.84$\pm$5.78 & 59.03$\pm$7.67 & 69.12$\pm$0.36 & 18.11$\pm$3.34 & 9.56$\pm$6.31 & 7.46$\pm$3.27 & 20.83$\pm$15.02 & 20.40$\pm$13.25 & 65.50$\pm$6.61 & 62.00$\pm$6.61 & 25.55$\pm$3.63 & 20.79$\pm$2.84\\
&  & BiomedCLIP & 60.47$\pm$3.71 & 60.42$\pm$2.95 & 69.28$\pm$1.42 & 18.82$\pm$3.35 & 10.14$\pm$11.34 & 8.63$\pm$5.70 & 15.28$\pm$16.84 & 18.53$\pm$11.31 & 56.99$\pm$9.52 & 67.13$\pm$5.72 & 20.38$\pm$2.13 & 29.01$\pm$2.68\\
&  & C2L & 57.03$\pm$1.56 & 51.39$\pm$1.96 & 69.26$\pm$0.02 & 15.66$\pm$4.73 & 12.82$\pm$10.23 & 9.56$\pm$2.52 & 8.33$\pm$0.00 & 9.56$\pm$2.02 & 55.83$\pm$7.13 & 61.89$\pm$10.58 & 29.32$\pm$0.15 & 24.99$\pm$8.86\\
&  & CLIP & 50.58$\pm$4.06 & 52.78$\pm$4.28 & 69.45$\pm$0.22 & 13.84$\pm$2.42 & 23.43$\pm$18.65 & 4.52$\pm$3.45 & 11.11$\pm$6.36 & 11.66$\pm$7.25 & 61.89$\pm$12.71 & 38.46$\pm$6.07 & 22.78$\pm$4.32 & 22.33$\pm$2.58\\
&  & DINOv2 & 50.38$\pm$2.22 & 53.47$\pm$3.93 & 74.38$\pm$6.31 & 19.57$\pm$4.32 & 17.83$\pm$12.45 & 10.77$\pm$5.50 & 6.94$\pm$4.81 & 7.58$\pm$3.59 & 55.24$\pm$9.09 & 39.74$\pm$7.39 & 22.34$\pm$10.64 & 27.45$\pm$0.43\\
&  & MedCLIP & 45.46$\pm$6.96 & 49.31$\pm$0.98 & 69.70$\pm$0.44 & 18.87$\pm$2.11 & 9.79$\pm$9.25 & 11.90$\pm$8.11 & 6.94$\pm$2.41 & 7.58$\pm$2.72 & 40.33$\pm$14.41 & 48.25$\pm$2.80 & 24.45$\pm$7.26 & 23.01$\pm$6.28\\
&  & MedLVM & 43.72$\pm$5.38 & 52.08$\pm$1.70 & 70.81$\pm$0.48 & 21.29$\pm$6.72 & 7.93$\pm$2.46 & 5.59$\pm$1.92 & 6.94$\pm$2.41 & 7.34$\pm$2.45 & 42.77$\pm$9.84 & 45.57$\pm$1.58 & 27.74$\pm$4.74 & 25.29$\pm$5.53\\
&  & MedMAE & 45.57$\pm$1.58 & 47.92$\pm$0.00 & 70.17$\pm$0.56 & 16.68$\pm$1.77 & 11.42$\pm$9.45 & 7.23$\pm$2.28 & 4.17$\pm$0.00 & 3.85$\pm$0.00 & 41.96$\pm$4.59 & 53.38$\pm$5.05 & 25.41$\pm$3.66 & 21.27$\pm$3.58\\
&  & MoCo-CXR & 45.31$\pm$10.21 & 52.08$\pm$2.95 & 69.62$\pm$0.27 & 17.81$\pm$3.50 & 12.94$\pm$11.04 & 6.35$\pm$6.44 & 9.72$\pm$6.36 & 11.31$\pm$6.54 & 38.34$\pm$13.47 & 51.28$\pm$8.11 & 18.55$\pm$2.40 & 21.22$\pm$6.15\\
&  & PubMedCLIP & 47.74$\pm$7.21 & 47.92$\pm$1.70 & 69.42$\pm$0.09 & 19.02$\pm$1.59 & 3.73$\pm$3.85 & 2.73$\pm$2.27 & 6.94$\pm$2.41 & 7.34$\pm$2.45 & 48.60$\pm$8.22 & 44.87$\pm$7.19 & 22.71$\pm$4.00 & 19.98$\pm$2.18\\

\cline{2-15}
  &\multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP & 56.36$\pm$0.00 & 66.67$\pm$0.00 & 88.44$\pm$0.00 & 26.92$\pm$0.00 & 33.21$\pm$0.00 & 7.53$\pm$0.00 & 4.17$\pm$0.00 & 97.06$\pm$0.00 & 72.27$\pm$0.00 & 39.06$\pm$0.00 & 23.20$\pm$0.00 & 30.72$\pm$0.00\\
&  & BLIP2 & 63.43$\pm$0.00 & 75.00$\pm$0.00 & 78.25$\pm$0.00 & 23.95$\pm$0.00 & 11.04$\pm$0.00 & 8.25$\pm$0.00 & 12.50$\pm$0.00 & 80.46$\pm$0.00 & 68.07$\pm$0.00 & 57.03$\pm$0.00 & 23.08$\pm$0.00 & 31.34$\pm$0.00\\
&  & BiomedCLIP & 91.78$\pm$1.54 & 84.03$\pm$2.41 & 57.67$\pm$6.37 & 21.46$\pm$1.75 & 5.42$\pm$0.82 & 1.98$\pm$0.93 & 5.56$\pm$4.81 & 94.52$\pm$2.59 & 89.64$\pm$1.28 & 95.05$\pm$1.19 & 21.80$\pm$1.10 & 21.77$\pm$1.54\\
&  & CLIP & 50.51$\pm$0.00 & 66.67$\pm$0.00 & 192.06$\pm$0.00 & 31.06$\pm$0.00 & 35.31$\pm$0.00 & 4.07$\pm$0.00 & 4.17$\pm$0.00 & 96.88$\pm$0.00 & 31.09$\pm$0.00 & 66.41$\pm$0.00 & 29.08$\pm$0.00 & 33.16$\pm$0.00\\
&  & MedCLIP & 51.18$\pm$7.29 & 68.06$\pm$1.20 & 66.94$\pm$2.50 & 17.24$\pm$3.96 & 15.61$\pm$3.91 & 4.96$\pm$2.19 & 6.94$\pm$2.41 & 92.30$\pm$4.18 & 56.02$\pm$14.95 & 48.70$\pm$11.96 & 22.47$\pm$0.75 & 27.42$\pm$2.73\\
&  & PubMedCLIP & 81.21$\pm$0.00 & 77.08$\pm$0.00 & 76.95$\pm$0.00 & 26.57$\pm$0.00 & 8.25$\pm$0.00 & 3.17$\pm$0.00 & 16.67$\pm$0.00 & 85.16$\pm$0.00 & 84.03$\pm$0.00 & 75.78$\pm$0.00 & 27.13$\pm$0.00 & 30.30$\pm$0.00\\
\cline{2-15}
 & \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP & 65.25$\pm$10.53 & 71.53$\pm$5.24 & 64.80$\pm$8.86 & 15.86$\pm$2.31 & 9.03$\pm$6.54 & 7.38$\pm$0.18 & 8.33$\pm$4.17 & 91.28$\pm$6.42 & 60.50$\pm$13.99 & 69.53$\pm$8.23 & 23.99$\pm$5.66 & 21.40$\pm$2.82\\
&  & BLIP2 & 66.60$\pm$15.35 & 69.44$\pm$3.18 & 62.49$\pm$3.90 & 17.69$\pm$1.77 & 12.41$\pm$8.95 & 2.60$\pm$2.05 & 6.94$\pm$2.41 & 91.70$\pm$4.73 & 72.83$\pm$17.83 & 60.42$\pm$17.01 & 23.32$\pm$2.28 & 20.88$\pm$3.56\\
&  & BiomedCLIP & 94.61$\pm$1.35 & 88.19$\pm$1.20 & 25.18$\pm$3.28 & 6.43$\pm$0.24 & 2.53$\pm$0.41 & 4.10$\pm$1.88 & 8.33$\pm$4.17 & 92.17$\pm$3.30 & 94.96$\pm$0.84 & 94.27$\pm$2.39 & 7.94$\pm$1.84 & 10.67$\pm$2.88\\
&  & CLIP & 64.51$\pm$14.24 & 68.75$\pm$3.61 & 65.51$\pm$8.40 & 21.79$\pm$4.29 & 11.79$\pm$9.19 & 5.69$\pm$0.61 & 5.56$\pm$2.41 & 93.91$\pm$5.46 & 62.75$\pm$22.71 & 65.89$\pm$7.09 & 27.04$\pm$4.02 & 28.49$\pm$3.78\\
&  & MedCLIP & 64.38$\pm$18.56 & 73.61$\pm$6.70 & 61.69$\pm$4.93 & 18.52$\pm$3.10 & 12.30$\pm$3.22 & 5.03$\pm$4.51 & 6.94$\pm$2.41 & 91.90$\pm$3.61 & 68.35$\pm$20.86 & 61.98$\pm$16.09 & 22.25$\pm$2.71 & 27.28$\pm$1.88\\
&  & PubMedCLIP & 87.00$\pm$2.37 & 78.47$\pm$2.41 & 47.34$\pm$1.97 & 15.74$\pm$3.49 & 3.07$\pm$1.16 & 4.45$\pm$3.79 & 25.00$\pm$0.00 & 71.99$\pm$2.84 & 88.52$\pm$4.63 & 86.72$\pm$2.07 & 18.83$\pm$2.92 & 20.16$\pm$3.60\\



\bottomrule
\end{tabular}
\end{threeparttable}
}
% \end{sidewaystable}
\end{table}

\begin{table}[htbp]

\centering
\caption{Classification results for CheXpert, FairVLMed10k, and GF3300 datasets, \textit{sex} as the sensitive attribute. All experiments are repeated three times and $\text{mean}\pm\text{std}$ are reported (\%).}    
\label{tab:full_res_cls_2}
% \adjustbox{width = \textwidth, height=}{
\resizebox*{0.6\textheight}{!}{
\begin{threeparttable}
\begin{tabular}{cccrrrrrrrrrrrrrr}
\toprule
\textbf{Dataset} & \textbf{Usage} & \textbf{Model}&\textbf{AUC}&\textbf{ACC}&\textbf{BCE}&\textbf{ECE}&$\Delta$\textbf{AUC}&$\Delta$\textbf{ECE}&\textbf{DP}&\textbf{EOD}&\textbf{AUC}$_{\text{Male}}$&\textbf{AUC}$_{\text{Female}}$&\textbf{ECE}$_{\text{Male}}$&\textbf{ECE}$_{\text{Female}}$ \\
\midrule
\multirow{23}{*}{{\rotatebox{90}{CheXpert}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP & 77.90$\pm$0.00 & 81.69$\pm$0.02 & 56.10$\pm$0.00 & 31.22$\pm$0.00 & 0.76$\pm$0.00 & 2.33$\pm$0.00 & 3.27$\pm$0.03 & 5.28$\pm$0.12 & 78.36$\pm$0.00 & 77.60$\pm$0.00 & 32.38$\pm$0.00 & 30.05$\pm$0.00\\
& & BLIP2 & 82.91$\pm$0.00 & 84.55$\pm$0.04 & 51.63$\pm$0.00 & 28.48$\pm$0.00 & 0.07$\pm$0.00 & 0.50$\pm$0.00 & 1.20$\pm$0.01 & 2.50$\pm$0.04 & 82.96$\pm$0.00 & 82.88$\pm$0.00 & 28.72$\pm$0.00 & 28.23$\pm$0.00\\
&  & BiomedCLIP & 83.60$\pm$0.00 & 84.81$\pm$0.02 & 50.30$\pm$0.00 & 26.29$\pm$0.00 & 0.77$\pm$0.00 & 1.59$\pm$0.01 & 1.72$\pm$0.02 & 2.16$\pm$0.02 & 83.23$\pm$0.00 & 84.01$\pm$0.00 & 27.08$\pm$0.01 & 25.49$\pm$0.00\\
&  & C2L & 81.88$\pm$0.00 & 84.94$\pm$0.00 & 65.53$\pm$0.00 & 38.26$\pm$0.00 & 1.45$\pm$0.00 & 0.11$\pm$0.00 & 0.04$\pm$0.00 & 2.00$\pm$0.00 & 81.18$\pm$0.00 & 82.63$\pm$0.00 & 38.31$\pm$0.00 & 38.20$\pm$0.00\\
& & CLIP & 76.61$\pm$0.00 & 81.01$\pm$0.00 & 59.32$\pm$0.00 & 34.16$\pm$0.00 & 0.91$\pm$0.00 & 2.65$\pm$0.00 & 2.71$\pm$0.02 & 4.83$\pm$0.05 & 77.25$\pm$0.00 & 76.34$\pm$0.00 & 35.49$\pm$0.00 & 32.84$\pm$0.00\\
&  & DINOv2 & 83.49$\pm$0.00 & 85.54$\pm$0.02 & 50.12$\pm$0.01 & 27.16$\pm$0.01 & 0.55$\pm$0.01 & 0.73$\pm$0.01 & 0.77$\pm$0.02 & 1.16$\pm$0.02 & 83.22$\pm$0.00 & 83.78$\pm$0.01 & 26.79$\pm$0.01 & 27.52$\pm$0.01\\
&  & MedCLIP & 89.77$\pm$0.00 & 89.33$\pm$0.02 & 43.04$\pm$0.14 & 21.90$\pm$0.09 & 1.11$\pm$0.00 & 0.23$\pm$0.01 & 1.04$\pm$0.01 & 2.77$\pm$0.04 & 89.21$\pm$0.00 & 90.32$\pm$0.00 & 21.78$\pm$0.10 & 22.01$\pm$0.09\\
&  & MedLVM & 83.15$\pm$0.01 & 86.44$\pm$0.01 & 51.27$\pm$0.02 & 28.03$\pm$0.01 & 0.76$\pm$0.00 & 0.81$\pm$0.02 & 1.21$\pm$0.03 & 1.40$\pm$0.06 & 82.78$\pm$0.01 & 83.54$\pm$0.01 & 28.44$\pm$0.00 & 27.63$\pm$0.02\\
&  & MedMAE & 84.39$\pm$0.00 & 86.30$\pm$0.45 & 51.14$\pm$0.01 & 28.67$\pm$0.01 & 1.08$\pm$0.00 & 0.00$\pm$0.00 & 1.63$\pm$0.01 & 2.05$\pm$0.07 & 83.87$\pm$0.00 & 84.96$\pm$0.00 & 28.67$\pm$0.00 & 28.67$\pm$0.01\\
&  & MoCo-CXR & 82.04$\pm$0.22 & 84.61$\pm$0.52 & 54.27$\pm$0.19 & 30.96$\pm$0.16 & 0.69$\pm$0.09 & 2.64$\pm$0.26 & 5.40$\pm$1.24 & 7.81$\pm$1.89 & 81.85$\pm$0.28 & 82.53$\pm$0.20 & 32.28$\pm$0.26 & 29.64$\pm$0.07\\
&  & PubMedCLIP & 78.51$\pm$0.00 & 83.92$\pm$0.17 & 56.81$\pm$0.00 & 32.38$\pm$0.00 & 0.38$\pm$0.00 & 2.33$\pm$0.00 & 2.13$\pm$0.03 & 3.77$\pm$0.14 & 78.81$\pm$0.00 & 78.43$\pm$0.00 & 33.55$\pm$0.00 & 31.22$\pm$0.00\\
\cline{2-15}
  & \multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP & 56.08$\pm$0.00 & 38.14$\pm$0.00 & 79.90$\pm$0.00 & 45.73$\pm$0.00 & 2.44$\pm$0.00 & 0.62$\pm$0.00 & 5.89$\pm$0.00 & 96.38$\pm$0.00 & 57.33$\pm$0.00 & 54.89$\pm$0.00 & 45.42$\pm$0.00 & 46.04$\pm$0.00\\
&  & BLIP2 & 63.65$\pm$0.00 & 64.14$\pm$1.41 & 49.85$\pm$0.00 & 25.71$\pm$0.00 & 3.57$\pm$0.01 & 0.27$\pm$0.00 & 9.11$\pm$0.08 & 88.19$\pm$0.35 & 61.87$\pm$0.00 & 65.44$\pm$0.01 & 25.58$\pm$0.00 & 25.85$\pm$0.00\\
&  & BiomedCLIP & 72.50$\pm$2.33 & 81.90$\pm$2.47 & 155.70$\pm$8.82 & 48.73$\pm$3.22 & 2.62$\pm$0.52 & 4.87$\pm$1.17 & 2.26$\pm$1.20 & 97.19$\pm$1.58 & 71.20$\pm$2.46 & 73.82$\pm$2.24 & 46.32$\pm$3.77 & 51.18$\pm$2.61\\
&  & CLIP & 54.05$\pm$0.00 & 29.15$\pm$0.00 & 120.38$\pm$0.00 & 61.80$\pm$0.00 & 1.61$\pm$0.00 & 0.66$\pm$0.00 & 2.97$\pm$0.00 & 96.74$\pm$0.00 & 53.18$\pm$0.00 & 54.79$\pm$0.00 & 61.47$\pm$0.00 & 62.13$\pm$0.00\\
&  & MedCLIP & 48.27$\pm$14.32 & 30.77$\pm$35.66 & 72.37$\pm$7.10 & 41.48$\pm$4.02 & 3.71$\pm$1.01 & 1.09$\pm$0.29 & 4.25$\pm$7.29 & 94.68$\pm$9.16 & 47.61$\pm$16.65 & 49.23$\pm$12.60 & 42.02$\pm$3.88 & 40.93$\pm$4.16\\
& & PubMedCLIP & 67.45$\pm$0.00 & 76.79$\pm$0.00 & 66.14$\pm$0.00 & 38.26$\pm$0.00 & 0.81$\pm$0.00 & 0.57$\pm$0.00 & 3.78$\pm$0.00 & 95.85$\pm$0.00 & 67.03$\pm$0.00 & 67.84$\pm$0.00 & 37.97$\pm$0.00 & 38.54$\pm$0.00\\
\cline{2-15}
  & \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP & 79.94$\pm$0.00 & 85.22$\pm$0.03 & 27.04$\pm$0.00 & 0.75$\pm$0.01 & 0.36$\pm$0.00 & 0.05$\pm$0.00 & 0.37$\pm$0.01 & 99.25$\pm$0.01 & 79.77$\pm$0.00 & 80.12$\pm$0.00 & 0.78$\pm$0.00 & 0.83$\pm$0.00\\
& & BLIP2 & 81.65$\pm$0.74 & 85.32$\pm$0.51 & 26.43$\pm$0.43 & 1.14$\pm$0.46 & 0.55$\pm$0.26 & 0.25$\pm$0.12 & 0.33$\pm$0.12 & 99.54$\pm$0.20 & 81.37$\pm$0.61 & 81.92$\pm$0.87 & 1.21$\pm$0.53 & 1.24$\pm$0.22\\
&  & BiomedCLIP & 84.07$\pm$0.00 & 86.06$\pm$0.31 & 25.20$\pm$0.00 & 0.68$\pm$0.01 & 0.88$\pm$0.00 & 0.37$\pm$0.07 & 1.51$\pm$0.09 & 98.00$\pm$0.07 & 83.65$\pm$0.00 & 84.53$\pm$0.00 & 0.53$\pm$0.03 & 0.91$\pm$0.04\\
& & CLIP & 81.23$\pm$0.00 & 84.83$\pm$0.03 & 26.52$\pm$0.00 & 0.76$\pm$0.01 & 0.16$\pm$0.00 & 0.14$\pm$0.01 & 0.87$\pm$0.04 & 98.00$\pm$0.04 & 81.17$\pm$0.00 & 81.32$\pm$0.00 & 0.85$\pm$0.00 & 0.72$\pm$0.01\\
&  & MedCLIP & 81.50$\pm$0.10 & 85.35$\pm$0.64 & 26.39$\pm$0.05 & 0.69$\pm$0.06 & 0.56$\pm$0.18 & 0.27$\pm$0.01 & 0.20$\pm$0.08 & 99.44$\pm$0.10 & 81.21$\pm$0.18 & 81.78$\pm$0.07 & 0.63$\pm$0.10 & 0.91$\pm$0.10\\
& & PubMedCLIP & 82.37$\pm$0.00 & 85.27$\pm$0.01 & 25.92$\pm$0.00 & 0.55$\pm$0.01 & 0.54$\pm$0.00 & 0.21$\pm$0.01 & 1.50$\pm$0.01 & 97.47$\pm$0.04 & 82.12$\pm$0.00 & 82.66$\pm$0.00 & 0.70$\pm$0.01 & 0.91$\pm$0.01\\

\midrule
\multirow{23}{*}{{\rotatebox{90}{FairVLMed10k}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP & 69.90$\pm$0.03 & 61.47$\pm$0.87 & 63.18$\pm$0.01 & 3.19$\pm$0.06 & 5.77$\pm$0.07 & 4.28$\pm$0.33 & 2.18$\pm$0.64 & 3.04$\pm$0.99 & 72.82$\pm$0.05 & 67.05$\pm$0.03 & 6.61$\pm$0.30 & 2.33$\pm$0.05\\
& & BLIP2 & 74.14$\pm$0.00 & 64.97$\pm$1.66 & 59.88$\pm$0.02 & 2.94$\pm$0.13 & 3.27$\pm$0.04 & 2.35$\pm$0.19 & 1.53$\pm$0.13 & 1.76$\pm$0.78 & 75.78$\pm$0.01 & 72.52$\pm$0.03 & 5.65$\pm$0.07 & 3.30$\pm$0.10\\
& & BiomedCLIP & 71.33$\pm$0.02 & 59.58$\pm$0.77 & 61.99$\pm$0.02 & 3.27$\pm$0.62 & 5.03$\pm$0.10 & 1.93$\pm$0.47 & 2.37$\pm$0.54 & 2.26$\pm$0.52 & 73.86$\pm$0.08 & 68.83$\pm$0.02 & 2.76$\pm$0.32 & 4.69$\pm$0.31\\
& & C2L & 69.66$\pm$0.01 & 60.02$\pm$0.05 & 66.33$\pm$0.01 & 10.84$\pm$0.07 & 3.15$\pm$0.01 & 1.96$\pm$0.30 & 3.09$\pm$0.11 & 2.96$\pm$0.11 & 71.24$\pm$0.02 & 68.09$\pm$0.01 & 12.10$\pm$0.15 & 10.14$\pm$0.10\\
& & CLIP & 68.47$\pm$0.06 & 63.12$\pm$0.26 & 64.23$\pm$0.02 & 5.77$\pm$0.15 & 4.26$\pm$0.02 & 1.64$\pm$0.74 & 3.78$\pm$0.64 & 3.57$\pm$0.64 & 70.51$\pm$0.07 & 66.25$\pm$0.06 & 7.09$\pm$0.48 & 5.44$\pm$0.47\\
& & DINOv2 & 76.63$\pm$0.05 & 66.02$\pm$1.03 & 57.33$\pm$0.02 & 2.87$\pm$0.35 & 1.45$\pm$0.11 & 0.51$\pm$0.49 & 1.49$\pm$0.23 & 1.46$\pm$0.08 & 77.34$\pm$0.04 & 75.89$\pm$0.10 & 3.86$\pm$0.04 & 3.56$\pm$0.54\\
& & MedCLIP & 72.44$\pm$0.09 & 63.90$\pm$1.23 & 62.05$\pm$0.04 & 5.57$\pm$0.14 & 4.94$\pm$0.09 & 2.18$\pm$0.61 & 3.28$\pm$0.63 & 3.06$\pm$0.60 & 74.91$\pm$0.10 & 69.98$\pm$0.11 & 7.34$\pm$0.25 & 5.16$\pm$0.40\\
& & MedLVM & 73.12$\pm$0.01 & 64.76$\pm$0.48 & 60.90$\pm$0.01 & 2.95$\pm$0.48 & 4.42$\pm$0.21 & 2.20$\pm$0.88 & 1.11$\pm$0.13 & 3.92$\pm$0.92 & 75.32$\pm$0.11 & 70.90$\pm$0.09 & 3.50$\pm$0.16 & 5.70$\pm$0.83\\
& & MedMAE & 68.72$\pm$0.01 & 60.92$\pm$0.38 & 64.29$\pm$0.01 & 4.73$\pm$0.14 & 2.17$\pm$0.06 & 3.00$\pm$0.14 & 3.51$\pm$0.74 & 3.35$\pm$0.73 & 69.76$\pm$0.04 & 67.59$\pm$0.03 & 6.50$\pm$0.04 & 3.50$\pm$0.15\\
& & MoCo-CXR & 69.22$\pm$0.45 & 61.72$\pm$0.82 & 64.26$\pm$0.25 & 5.52$\pm$0.49 & 3.70$\pm$1.08 & 3.01$\pm$0.21 & 3.44$\pm$1.16 & 3.51$\pm$1.00 & 70.99$\pm$0.84 & 67.29$\pm$0.53 & 7.48$\pm$0.25 & 4.48$\pm$0.38\\
& & PubMedCLIP & 67.84$\pm$0.07 & 60.94$\pm$0.08 & 64.44$\pm$0.02 & 5.38$\pm$0.23 & 4.55$\pm$0.02 & 2.30$\pm$0.56 & 5.23$\pm$0.07 & 5.05$\pm$0.06 & 70.08$\pm$0.07 & 65.53$\pm$0.07 & 6.76$\pm$0.57 & 4.46$\pm$0.12\\

\cline{2-15}
  & \multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}}& BLIP & 44.44$\pm$0.00 & 51.49$\pm$0.00 & 81.84$\pm$0.00 & 19.67$\pm$0.00 & 4.48$\pm$0.00 & 3.13$\pm$0.00 & 0.00$\pm$0.00 & 99.54$\pm$0.00 & 42.18$\pm$0.00 & 46.67$\pm$0.00 & 21.20$\pm$0.00 & 18.06$\pm$0.00\\
&& BLIP2 & 43.83$\pm$0.01 & 51.32$\pm$0.00 & 78.02$\pm$0.00 & 18.05$\pm$0.00 & 2.95$\pm$0.01 & 0.61$\pm$0.04 & 0.11$\pm$0.00 & 99.89$\pm$0.00 & 42.47$\pm$0.01 & 45.42$\pm$0.01 & 18.23$\pm$0.00 & 18.84$\pm$0.04\\
& & BiomedCLIP & 54.33$\pm$2.39 & 51.32$\pm$0.00 & 110.30$\pm$25.16 & 29.48$\pm$9.47 & 2.12$\pm$1.58 & 2.07$\pm$1.42 & 0.11$\pm$0.00 & 99.89$\pm$0.00 & 53.24$\pm$2.94 & 55.37$\pm$1.89 & 30.59$\pm$10.08 & 28.52$\pm$8.93\\
& & CLIP & 60.19$\pm$0.00 & 52.52$\pm$0.00 & 72.61$\pm$0.00 & 15.13$\pm$0.00 & 0.28$\pm$0.00 & 0.40$\pm$0.00 & 0.00$\pm$0.00 & 99.51$\pm$0.00 & 60.04$\pm$0.00 & 60.33$\pm$0.00 & 15.03$\pm$0.00 & 15.43$\pm$0.00\\
& & MedCLIP & 54.23$\pm$6.33 & 51.49$\pm$0.15 & 69.91$\pm$0.27 & 6.51$\pm$2.53 & 1.91$\pm$0.97 & 0.37$\pm$0.54 & 0.15$\pm$0.07 & 99.77$\pm$0.11 & 54.30$\pm$7.19 & 54.20$\pm$5.65 & 7.39$\pm$3.30 & 7.10$\pm$2.69\\
& & PubMedCLIP & 50.02$\pm$0.00 & 51.32$\pm$0.00 & 74.95$\pm$0.00 & 14.49$\pm$0.00 & 0.49$\pm$0.00 & 1.20$\pm$0.00 & 0.11$\pm$0.00 & 99.89$\pm$0.00 & 49.81$\pm$0.00 & 50.30$\pm$0.00 & 13.84$\pm$0.00 & 15.04$\pm$0.00\\

\cline{2-15}
  &\multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP & 75.35$\pm$0.01 & 67.60$\pm$0.35 & 58.98$\pm$0.01 & 1.62$\pm$0.04 & 3.81$\pm$0.01 & 0.23$\pm$0.19 & 0.61$\pm$0.13 & 96.02$\pm$0.36 & 77.29$\pm$0.02 & 73.48$\pm$0.01 & 3.64$\pm$0.21 & 3.41$\pm$0.05\\
&& BLIP2 & 73.28$\pm$0.13 & 67.16$\pm$0.44 & 60.80$\pm$0.10 & 3.48$\pm$0.49 & 3.14$\pm$0.42 & 0.78$\pm$0.66 & 1.49$\pm$0.30 & 98.16$\pm$0.49 & 74.81$\pm$0.33 & 71.67$\pm$0.12 & 4.66$\pm$0.16 & 4.88$\pm$1.15\\
& & BiomedCLIP & 72.62$\pm$0.08 & 65.71$\pm$0.75 & 61.15$\pm$0.08 & 3.53$\pm$0.05 & 3.05$\pm$0.16 & 0.73$\pm$0.61 & 2.48$\pm$0.17 & 97.73$\pm$0.17 & 74.11$\pm$0.04 & 71.06$\pm$0.16 & 4.51$\pm$0.29 & 3.78$\pm$0.35\\
& & CLIP & 74.38$\pm$0.02 & 65.23$\pm$0.06 & 59.60$\pm$0.02 & 2.83$\pm$0.29 & 1.91$\pm$0.05 & 1.40$\pm$0.31 & 0.84$\pm$0.24 & 97.28$\pm$0.18 & 75.32$\pm$0.05 & 73.41$\pm$0.00 & 4.28$\pm$0.12 & 2.88$\pm$0.24\\
& & MedCLIP & 75.29$\pm$0.41 & 65.77$\pm$2.55 & 58.94$\pm$0.34 & 2.85$\pm$0.91 & 3.51$\pm$0.15 & 0.72$\pm$0.21 & 1.91$\pm$0.13 & 97.99$\pm$0.16 & 77.02$\pm$0.33 & 73.51$\pm$0.47 & 4.24$\pm$0.77 & 3.52$\pm$0.59\\
& & PubMedCLIP & 73.69$\pm$0.00 & 66.65$\pm$0.34 & 60.37$\pm$0.01 & 2.36$\pm$0.06 & 3.94$\pm$0.01 & 1.47$\pm$0.12 & 2.52$\pm$0.20 & 97.34$\pm$0.17 & 75.60$\pm$0.01 & 71.66$\pm$0.01 & 3.36$\pm$0.02 & 4.83$\pm$0.11\\
\midrule
\multirow{23}{*}{{\rotatebox{90}{GF3300}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP & 77.45$\pm$0.16 & 69.47$\pm$0.21 & 57.01$\pm$0.20 & 8.48$\pm$0.80 & 2.74$\pm$0.24 & 2.30$\pm$1.56 & 4.15$\pm$0.85 & 5.28$\pm$0.84 & 78.92$\pm$0.16 & 76.18$\pm$0.22 & 8.73$\pm$1.62 & 10.62$\pm$0.28\\
& & BLIP2 & 80.09$\pm$0.08 & 70.54$\pm$1.67 & 53.81$\pm$0.06 & 7.61$\pm$0.50 & 1.64$\pm$0.22 & 3.99$\pm$0.88 & 3.59$\pm$2.72 & 4.84$\pm$2.85 & 81.00$\pm$0.05 & 79.36$\pm$0.23 & 9.88$\pm$0.59 & 5.89$\pm$0.31\\
& & BiomedCLIP & 80.13$\pm$0.18 & 75.25$\pm$0.50 & 52.97$\pm$0.34 & 7.67$\pm$0.38 & 2.44$\pm$0.31 & 2.62$\pm$0.31 & 5.16$\pm$0.70 & 6.63$\pm$0.68 & 81.64$\pm$0.29 & 79.19$\pm$0.08 & 9.94$\pm$0.43 & 7.32$\pm$0.54\\
& & C2L & 82.33$\pm$0.21 & 72.28$\pm$0.08 & 63.19$\pm$0.27 & 20.46$\pm$0.01 & 0.66$\pm$0.39 & 0.65$\pm$0.24 & 1.01$\pm$0.58 & 2.35$\pm$0.55 & 82.60$\pm$0.46 & 82.08$\pm$0.17 & 21.20$\pm$0.45 & 21.23$\pm$0.23\\
& & CLIP & 80.23$\pm$0.15 & 74.02$\pm$0.16 & 58.20$\pm$0.02 & 12.55$\pm$0.02 & 2.22$\pm$0.14 & 1.42$\pm$0.31 & 7.41$\pm$0.00 & 8.96$\pm$0.00 & 79.23$\pm$0.23 & 81.45$\pm$0.09 & 12.65$\pm$0.15 & 14.07$\pm$0.40\\
&& DINOv2 & 80.79$\pm$0.45 & 74.24$\pm$0.24 & 53.02$\pm$0.49 & 6.64$\pm$0.23 & 1.67$\pm$0.24 & 3.77$\pm$0.83 & 2.92$\pm$0.97 & 1.96$\pm$0.83 & 81.69$\pm$0.63 & 80.02$\pm$0.39 & 9.14$\pm$0.25 & 5.38$\pm$0.92\\
& & MedCLIP & 76.39$\pm$0.15 & 67.23$\pm$0.40 & 62.09$\pm$0.00 & 10.43$\pm$0.17 & 1.58$\pm$0.03 & 3.74$\pm$0.94 & 1.23$\pm$0.19 & 2.82$\pm$0.81 & 77.26$\pm$0.15 & 75.68$\pm$0.12 & 12.63$\pm$0.45 & 8.89$\pm$0.31\\
& & MedLVM & 82.54$\pm$0.03 & 75.31$\pm$0.40 & 49.73$\pm$0.07 & 5.61$\pm$0.13 & 1.42$\pm$0.04 & 0.54$\pm$0.60 & 3.03$\pm$0.58 & 4.65$\pm$0.48 & 83.40$\pm$0.03 & 81.98$\pm$0.07 & 7.71$\pm$0.19 & 7.17$\pm$0.30\\
& & MedMAE & 80.60$\pm$0.01 & 71.04$\pm$0.00 & 54.78$\pm$0.04 & 10.65$\pm$0.14 & 2.14$\pm$0.04 & 2.51$\pm$0.51 & 6.62$\pm$0.39 & 7.95$\pm$0.38 & 81.73$\pm$0.02 & 79.59$\pm$0.05 & 12.72$\pm$0.16 & 10.21$\pm$0.26\\
&& MoCo-CXR & 82.34$\pm$0.19 & 75.42$\pm$0.48 & 55.42$\pm$0.81 & 12.84$\pm$1.52 & 0.93$\pm$0.11 & 1.98$\pm$0.99 & 3.48$\pm$0.39 & 5.03$\pm$0.39 & 82.51$\pm$0.75 & 82.28$\pm$0.36 & 13.74$\pm$0.24 & 12.31$\pm$1.83\\
& & PubMedCLIP & 78.40$\pm$0.01 & 64.42$\pm$0.21 & 57.33$\pm$0.03 & 11.86$\pm$0.17 & 2.86$\pm$0.02 & 3.72$\pm$1.22 & 5.27$\pm$0.19 & 6.12$\pm$0.18 & 79.97$\pm$0.01 & 77.11$\pm$0.01 & 13.84$\pm$0.47 & 10.11$\pm$0.53\\

\cline{2-15}
 & \multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP & 42.47$\pm$0.00 & 50.84$\pm$0.00 & 107.25$\pm$0.00 & 33.83$\pm$0.00 & 0.95$\pm$0.00 & 0.36$\pm$0.00 & 0.34$\pm$0.00 & 99.68$\pm$0.00 & 41.88$\pm$0.00 & 42.83$\pm$0.00 & 34.24$\pm$0.00 & 33.88$\pm$0.00\\
& & BLIP2 & 42.75$\pm$0.01 & 50.84$\pm$0.00 & 81.84$\pm$0.01 & 20.87$\pm$0.00 & 1.31$\pm$0.07 & 3.09$\pm$0.00 & 0.34$\pm$0.00 & 99.68$\pm$0.00 & 43.44$\pm$0.05 & 42.13$\pm$0.02 & 19.26$\pm$0.00 & 22.35$\pm$0.00\\
& & BiomedCLIP & 56.65$\pm$1.90 & 50.84$\pm$0.00 & 214.87$\pm$67.59 & 43.02$\pm$5.68 & 1.98$\pm$1.51 & 1.82$\pm$0.79 & 0.34$\pm$0.00 & 99.67$\pm$0.01 & 55.73$\pm$2.50 & 57.72$\pm$1.65 & 44.18$\pm$6.17 & 42.36$\pm$5.51\\
& & CLIP & 70.64$\pm$0.00 & 62.79$\pm$0.00 & 215.28$\pm$0.00 & 47.68$\pm$0.00 & 1.63$\pm$0.00 & 3.05$\pm$0.00 & 3.37$\pm$0.00 & 95.83$\pm$0.00 & 71.69$\pm$0.00 & 70.06$\pm$0.00 & 49.17$\pm$0.00 & 46.12$\pm$0.00\\
& & MedCLIP & 46.27$\pm$16.46 & 54.32$\pm$5.88 & 70.70$\pm$2.52 & 12.52$\pm$4.54 & 4.42$\pm$3.74 & 2.74$\pm$3.31 & 2.81$\pm$3.99 & 96.97$\pm$4.38 & 44.98$\pm$19.35 & 47.54$\pm$13.85 & 13.92$\pm$6.77 & 11.81$\pm$2.90\\
& & PubMedCLIP & 39.87$\pm$0.00 & 50.84$\pm$0.00 & 87.67$\pm$0.00 & 23.90$\pm$0.00 & 3.31$\pm$0.00 & 2.31$\pm$0.00 & 0.34$\pm$0.00 & 99.68$\pm$0.00 & 38.22$\pm$0.00 & 41.53$\pm$0.00 & 25.97$\pm$0.00 & 23.66$\pm$0.00\\

\cline{2-15}
 & \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP & 83.52$\pm$0.03 & 74.80$\pm$0.26 & 49.41$\pm$0.04 & 4.93$\pm$0.49 & 1.65$\pm$0.09 & 2.84$\pm$0.38 & 3.37$\pm$0.34 & 95.44$\pm$0.68 & 84.14$\pm$0.07 & 82.49$\pm$0.03 & 6.96$\pm$0.17 & 4.13$\pm$0.42\\
& & BLIP2 & 71.36$\pm$7.48 & 59.93$\pm$9.50 & 61.88$\pm$6.75 & 6.89$\pm$2.12 & 5.85$\pm$3.24 & 5.04$\pm$2.04 & 2.58$\pm$0.19 & 97.70$\pm$0.75 & 74.45$\pm$5.79 & 68.59$\pm$9.02 & 10.44$\pm$2.15 & 5.40$\pm$0.38\\
& & BiomedCLIP & 83.12$\pm$0.14 & 74.97$\pm$2.04 & 49.77$\pm$0.16 & 4.72$\pm$1.86 & 3.15$\pm$0.41 & 3.07$\pm$0.84 & 2.36$\pm$2.05 & 94.91$\pm$1.79 & 81.64$\pm$0.28 & 84.79$\pm$0.16 & 5.88$\pm$1.24 & 7.17$\pm$2.78\\
&& CLIP & 82.82$\pm$0.03 & 72.95$\pm$0.26 & 50.19$\pm$0.04 & 6.50$\pm$0.44 & 0.46$\pm$0.07 & 0.89$\pm$0.24 & 3.03$\pm$0.89 & 98.15$\pm$0.86 & 83.02$\pm$0.01 & 82.57$\pm$0.07 & 7.36$\pm$0.54 & 6.47$\pm$0.72\\
& & MedCLIP & 81.93$\pm$0.44 & 72.62$\pm$0.83 & 51.66$\pm$0.38 & 5.95$\pm$1.88 & 1.23$\pm$0.36 & 3.53$\pm$2.79 & 3.25$\pm$1.85 & 95.38$\pm$1.87 & 82.60$\pm$0.64 & 81.38$\pm$0.34 & 8.29$\pm$1.60 & 4.75$\pm$1.20\\
& & PubMedCLIP & 80.57$\pm$0.03 & 71.21$\pm$0.29 & 52.70$\pm$0.04 & 4.32$\pm$0.23 & 2.10$\pm$0.08 & 1.91$\pm$0.61 & 5.39$\pm$1.21 & 93.34$\pm$1.26 & 81.75$\pm$0.05 & 79.64$\pm$0.04 & 6.76$\pm$0.28 & 4.86$\pm$0.60\\



\bottomrule
\end{tabular}
\end{threeparttable}
}
% \end{sidewaystable}
\end{table}

\begin{table}[htbp]

\centering
\caption{Classification results for HAM10000, MIMIC-CXR, and PAPILA datasets, \textit{sex} as the sensitive attribute. All experiments are repeated three times and $\text{mean}\pm\text{std}$ are reported (\%).}
\label{tab:full_res_cls_3}
% \adjustbox{width = \textwidth, height=}{
\resizebox*{0.6\textheight}{!}{
\begin{threeparttable}
\begin{tabular}{cccrrrrrrrrrrrrrr}
\toprule
\textbf{Dataset} & \textbf{Usage} & \textbf{Model}&\textbf{AUC}&\textbf{ACC}&\textbf{BCE}&\textbf{ECE}&$\Delta$\textbf{AUC}&$\Delta$\textbf{ECE}&\textbf{DP}&\textbf{EOD}&\textbf{AUC}$_{\text{Male}}$&\textbf{AUC}$_{\text{Female}}$&\textbf{ECE}$_{\text{Male}}$&\textbf{ECE}$_{\text{Female}}$ \\
\midrule
\multirow{23}{*}{{\rotatebox{90}{HAM10000}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}}  & BLIP & 86.25$\pm$0.01 & 81.10$\pm$0.11 & 48.81$\pm$0.04 & 24.26$\pm$0.04 & 0.11$\pm$0.06 & 1.58$\pm$0.05 & 11.71$\pm$0.35 & 7.75$\pm$0.87 & 85.77$\pm$0.04 & 85.85$\pm$0.08 & 23.47$\pm$0.02 & 25.05$\pm$0.06\\
& & BLIP2 & 90.14$\pm$0.04 & 86.78$\pm$0.53 & 43.54$\pm$0.04 & 20.72$\pm$0.05 & 2.34$\pm$0.06 & 0.66$\pm$0.06 & 9.74$\pm$0.61 & 12.05$\pm$0.19 & 90.79$\pm$0.04 & 88.44$\pm$0.07 & 21.04$\pm$0.05 & 20.39$\pm$0.07\\
& & BiomedCLIP & 85.70$\pm$0.08 & 80.99$\pm$0.75 & 49.13$\pm$0.11 & 21.21$\pm$0.14 & 2.83$\pm$0.08 & 0.78$\pm$0.10 & 8.18$\pm$0.83 & 7.92$\pm$1.34 & 86.52$\pm$0.14 & 83.69$\pm$0.10 & 20.81$\pm$0.14 & 21.60$\pm$0.16\\
&& C2L & 78.72$\pm$0.02 & 71.42$\pm$1.91 & 62.84$\pm$0.30 & 33.12$\pm$0.21 & 3.06$\pm$0.12 & 6.01$\pm$0.04 & 8.73$\pm$0.57 & 8.59$\pm$0.75 & 79.43$\pm$0.06 & 76.37$\pm$0.06 & 30.11$\pm$0.19 & 36.12$\pm$0.23\\
& & CLIP & 84.85$\pm$0.06 & 82.64$\pm$1.16 & 51.81$\pm$0.07 & 26.05$\pm$0.04 & 0.23$\pm$0.05 & 1.80$\pm$0.01 & 9.64$\pm$1.80 & 6.95$\pm$1.63 & 84.14$\pm$0.08 & 84.37$\pm$0.08 & 25.15$\pm$0.03 & 26.95$\pm$0.04\\
& & DINOv2 & 85.88$\pm$0.11 & 84.02$\pm$0.55 & 46.19$\pm$0.05 & 20.65$\pm$0.06 & 3.48$\pm$0.15 & 0.22$\pm$0.02 & 9.45$\pm$0.11 & 14.50$\pm$1.40 & 87.03$\pm$0.06 & 83.54$\pm$0.19 & 20.76$\pm$0.05 & 20.54$\pm$0.06\\
& & MedCLIP & 81.09$\pm$0.22 & 77.45$\pm$1.21 & 56.21$\pm$0.09 & 28.60$\pm$0.10 & 6.44$\pm$0.27 & 3.01$\pm$0.20 & 9.81$\pm$1.93 & 13.06$\pm$3.18 & 83.11$\pm$0.29 & 76.66$\pm$0.09 & 27.09$\pm$0.15 & 30.10$\pm$0.10\\
& & MedLVM & 87.26$\pm$0.06 & 85.57$\pm$0.38 & 47.50$\pm$0.10 & 22.95$\pm$0.07 & 2.80$\pm$0.07 & 0.11$\pm$0.04 & 13.28$\pm$0.17 & 18.11$\pm$0.54 & 87.99$\pm$0.06 & 85.19$\pm$0.13 & 22.89$\pm$0.07 & 23.01$\pm$0.07\\
& & MedMAE & 85.34$\pm$0.03 & 82.88$\pm$0.32 & 50.20$\pm$0.01 & 24.97$\pm$0.00 & 4.78$\pm$0.03 & 2.91$\pm$0.03 & 9.16$\pm$0.07 & 14.23$\pm$0.45 & 86.77$\pm$0.02 & 81.99$\pm$0.04 & 23.51$\pm$0.01 & 26.42$\pm$0.02\\
& & MoCo-CXR & 82.92$\pm$1.10 & 79.27$\pm$1.43 & 55.62$\pm$0.85 & 28.64$\pm$0.37 & 5.97$\pm$1.78 & 1.15$\pm$0.65 & 12.42$\pm$1.15 & 16.73$\pm$2.81 & 84.87$\pm$0.64 & 78.90$\pm$2.14 & 28.07$\pm$0.28 & 29.22$\pm$0.58\\
& & PubMedCLIP & 85.89$\pm$0.09 & 79.90$\pm$0.16 & 51.26$\pm$0.08 & 26.13$\pm$0.03 & 1.93$\pm$0.01 & 2.25$\pm$0.05 & 11.98$\pm$0.34 & 7.24$\pm$0.27 & 84.62$\pm$0.10 & 86.55$\pm$0.09 & 25.00$\pm$0.02 & 27.25$\pm$0.05\\
\cline{2-15}
  &\multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP & 42.85$\pm$0.00 & 17.56$\pm$0.00 & 70.89$\pm$0.00 & 33.43$\pm$0.00 & 4.59$\pm$0.00 & 13.28$\pm$0.00 & 3.88$\pm$0.00 & 96.85$\pm$0.00 & 46.79$\pm$0.00 & 42.20$\pm$0.00 & 26.78$\pm$0.00 & 40.06$\pm$0.00\\
& & BLIP2 & 44.36$\pm$0.01 & 14.47$\pm$0.00 & 59.90$\pm$0.00 & 25.68$\pm$0.00 & 0.73$\pm$0.00 & 9.76$\pm$0.00 & 0.11$\pm$0.00 & 99.70$\pm$0.00 & 45.42$\pm$0.01 & 44.69$\pm$0.00 & 21.01$\pm$0.00 & 30.77$\pm$0.00\\
& & BiomedCLIP & 67.26$\pm$5.49 & 64.84$\pm$7.75 & 112.30$\pm$31.30 & 45.56$\pm$8.66 & 1.19$\pm$0.25 & 5.89$\pm$1.59 & 3.61$\pm$3.27 & 96.90$\pm$1.49 & 66.71$\pm$5.34 & 67.90$\pm$5.42 & 42.61$\pm$7.87 & 48.49$\pm$9.44\\
& & CLIP & 72.05$\pm$0.00 & 74.16$\pm$0.00 & 73.86$\pm$0.00 & 37.55$\pm$0.00 & 5.19$\pm$0.00 & 5.03$\pm$0.00 & 6.16$\pm$0.00 & 91.98$\pm$0.00 & 73.58$\pm$0.00 & 68.39$\pm$0.00 & 35.03$\pm$0.00 & 40.06$\pm$0.00\\
& & MedCLIP & 54.11$\pm$11.53 & 32.91$\pm$29.79 & 69.05$\pm$4.07 & 35.16$\pm$3.24 & 8.29$\pm$3.72 & 7.87$\pm$0.86 & 1.81$\pm$1.91 & 97.92$\pm$2.10 & 56.11$\pm$13.81 & 51.34$\pm$9.71 & 31.23$\pm$3.56 & 39.10$\pm$2.91\\
& & PubMedCLIP & 62.38$\pm$0.00 & 63.78$\pm$0.00 & 99.15$\pm$0.00 & 50.08$\pm$0.00 & 8.29$\pm$0.00 & 2.05$\pm$0.00 & 16.58$\pm$0.00 & 79.98$\pm$0.00 & 64.06$\pm$0.00 & 55.77$\pm$0.00 & 49.06$\pm$0.00 & 51.11$\pm$0.00\\

\cline{2-15}
  & \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP & 87.44$\pm$0.01 & 82.35$\pm$0.11 & 28.60$\pm$0.01 & 1.64$\pm$0.06 & 2.12$\pm$0.02 & 0.39$\pm$0.08 & 10.53$\pm$0.23 & 89.39$\pm$0.43 & 87.88$\pm$0.01 & 85.76$\pm$0.01 & 2.80$\pm$0.18 & 2.40$\pm$0.10\\
& & BLIP2 & 86.97$\pm$1.26 & 81.00$\pm$1.05 & 29.05$\pm$1.23 & 2.10$\pm$0.39 & 2.55$\pm$0.77 & 0.70$\pm$0.48 & 8.15$\pm$1.09 & 91.93$\pm$0.28 & 87.65$\pm$1.54 & 85.09$\pm$0.78 & 3.48$\pm$0.44 & 2.78$\pm$0.18\\
& & BiomedCLIP & 87.12$\pm$0.03 & 84.63$\pm$3.38 & 28.89$\pm$0.02 & 1.92$\pm$0.09 & 0.79$\pm$0.16 & 1.32$\pm$0.67 & 6.98$\pm$1.37 & 94.58$\pm$0.98 & 87.16$\pm$0.11 & 86.37$\pm$0.06 & 3.80$\pm$0.62 & 2.47$\pm$0.10\\
& & CLIP & 87.94$\pm$0.00 & 84.17$\pm$0.11 & 28.19$\pm$0.00 & 1.58$\pm$0.04 & 2.84$\pm$0.01 & 0.43$\pm$0.09 & 7.39$\pm$0.06 & 91.13$\pm$0.04 & 88.83$\pm$0.00 & 86.00$\pm$0.01 & 3.41$\pm$0.05 & 2.98$\pm$0.05\\
& & MedCLIP & 84.80$\pm$0.06 & 83.80$\pm$0.75 & 30.77$\pm$0.08 & 1.84$\pm$0.32 & 0.67$\pm$0.20 & 0.86$\pm$0.20 & 10.70$\pm$1.53 & 89.25$\pm$3.01 & 84.12$\pm$0.27 & 84.49$\pm$0.44 & 3.47$\pm$0.23 & 2.61$\pm$0.28\\
& & PubMedCLIP & 86.93$\pm$0.01 & 83.25$\pm$0.11 & 29.59$\pm$0.01 & 2.79$\pm$0.09 & 2.03$\pm$0.03 & 1.27$\pm$0.06 & 11.30$\pm$0.17 & 89.60$\pm$0.71 & 87.37$\pm$0.02 & 85.34$\pm$0.01 & 4.14$\pm$0.11 & 2.87$\pm$0.05\\
\midrule
\multirow{23}{*}{{\rotatebox{90}{MIMIC-CXR}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP & 76.14$\pm$0.00 & 68.45$\pm$0.01 & 59.08$\pm$0.00 & 10.34$\pm$0.00 & 0.99$\pm$0.00 & 4.67$\pm$0.00 & 4.16$\pm$0.01 & 1.97$\pm$0.01 & 75.60$\pm$0.00 & 76.59$\pm$0.00 & 12.85$\pm$0.00 & 8.18$\pm$0.00\\
& & BLIP2 & 80.79$\pm$0.00 & 73.45$\pm$0.00 & 54.21$\pm$0.00 & 9.30$\pm$0.00 & 1.84$\pm$0.00 & 1.47$\pm$0.00 & 8.23$\pm$0.01 & 5.54$\pm$0.01 & 79.69$\pm$0.00 & 81.53$\pm$0.00 & 10.04$\pm$0.00 & 8.57$\pm$0.00\\
& & BiomedCLIP & 81.25$\pm$0.00 & 73.58$\pm$0.45 & 53.18$\pm$0.00 & 8.53$\pm$0.00 & 1.58$\pm$0.00 & 3.91$\pm$0.00 & 3.25$\pm$0.12 & 1.17$\pm$0.14 & 80.39$\pm$0.00 & 81.97$\pm$0.00 & 10.49$\pm$0.00 & 6.58$\pm$0.00\\
& & C2L & 80.20$\pm$0.00 & 72.12$\pm$0.00 & 66.91$\pm$0.00 & 22.24$\pm$0.00 & 1.53$\pm$0.00 & 2.22$\pm$0.00 & 5.06$\pm$0.00 & 2.61$\pm$0.00 & 79.30$\pm$0.00 & 80.83$\pm$0.00 & 23.49$\pm$0.00 & 21.27$\pm$0.00\\
& & CLIP & 74.83$\pm$0.00 & 66.41$\pm$0.01 & 61.69$\pm$0.00 & 11.95$\pm$0.00 & 2.48$\pm$0.00 & 2.90$\pm$0.01 & 4.27$\pm$0.01 & 2.52$\pm$0.00 & 73.39$\pm$0.00 & 75.87$\pm$0.00 & 13.49$\pm$0.00 & 10.60$\pm$0.01\\
& & DINOv2 & 81.00$\pm$0.00 & 72.68$\pm$0.00 & 53.90$\pm$0.00 & 9.13$\pm$0.00 & 1.48$\pm$0.00 & 1.44$\pm$0.00 & 8.10$\pm$0.01 & 5.32$\pm$0.01 & 80.10$\pm$0.00 & 81.58$\pm$0.00 & 9.85$\pm$0.00 & 8.41$\pm$0.00\\
& & MedCLIP & 89.38$\pm$0.00 & 82.23$\pm$0.01 & 41.98$\pm$0.01 & 7.61$\pm$0.01 & 0.27$\pm$0.00 & 0.22$\pm$0.00 & 7.57$\pm$0.01 & 3.64$\pm$0.01 & 89.17$\pm$0.00 & 89.44$\pm$0.00 & 7.72$\pm$0.01 & 7.50$\pm$0.01\\
&& MedLVM & 80.68$\pm$0.00 & 72.06$\pm$0.03 & 54.33$\pm$0.00 & 9.37$\pm$0.01 & 1.60$\pm$0.00 & 2.39$\pm$0.00 & 7.06$\pm$0.02 & 4.41$\pm$0.02 & 79.72$\pm$0.00 & 81.32$\pm$0.00 & 10.57$\pm$0.00 & 8.17$\pm$0.01\\
&& MedMAE & 80.73$\pm$0.00 & 72.88$\pm$0.09 & 54.65$\pm$0.00 & 9.97$\pm$0.00 & 1.83$\pm$0.00 & 1.41$\pm$0.01 & 6.91$\pm$0.02 & 4.35$\pm$0.01 & 79.66$\pm$0.00 & 81.50$\pm$0.00 & 10.69$\pm$0.01 & 9.28$\pm$0.01\\
&& MoCo-CXR & 79.50$\pm$0.37 & 72.07$\pm$0.57 & 56.87$\pm$0.33 & 10.92$\pm$0.33 & 1.45$\pm$0.10 & 2.94$\pm$0.18 & 2.50$\pm$1.74 & 1.39$\pm$0.47 & 78.77$\pm$0.37 & 80.22$\pm$0.43 & 12.94$\pm$0.41 & 10.00$\pm$0.37\\
& & PubMedCLIP & 77.46$\pm$0.00 & 70.43$\pm$0.00 & 58.64$\pm$0.00 & 10.75$\pm$0.00 & 1.67$\pm$0.00 & 3.03$\pm$0.00 & 5.68$\pm$0.00 & 3.33$\pm$0.00 & 76.47$\pm$0.00 & 78.14$\pm$0.00 & 12.49$\pm$0.00 & 9.45$\pm$0.00\\

\cline{2-15}
 & \multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP & 52.54$\pm$0.00 & 39.07$\pm$0.00 & 73.32$\pm$0.00 & 18.43$\pm$0.00 & 0.63$\pm$0.00 & 4.09$\pm$0.00 & 1.55$\pm$0.00 & 98.62$\pm$0.00 & 51.51$\pm$0.00 & 52.15$\pm$0.00 & 20.47$\pm$0.00 & 16.38$\pm$0.00\\
& & BLIP2 & 58.68$\pm$0.00 & 40.84$\pm$0.00 & 65.72$\pm$0.00 & 3.84$\pm$0.00 & 5.41$\pm$0.00 & 1.25$\pm$0.00 & 3.48$\pm$0.00 & 96.69$\pm$0.00 & 55.32$\pm$0.00 & 60.73$\pm$0.00 & 5.73$\pm$0.00 & 4.48$\pm$0.00\\
& & BiomedCLIP & 64.97$\pm$2.11 & 49.02$\pm$2.59 & 137.02$\pm$13.53 & 32.02$\pm$2.62 & 0.70$\pm$0.65 & 0.60$\pm$0.43 & 7.38$\pm$1.46 & 93.70$\pm$1.26 & 64.36$\pm$1.82 & 65.06$\pm$2.38 & 32.33$\pm$2.82 & 31.74$\pm$2.45\\
& & CLIP & 54.08$\pm$0.00 & 37.87$\pm$0.00 & 97.19$\pm$0.00 & 36.55$\pm$0.00 & 0.71$\pm$0.00 & 5.23$\pm$0.00 & 0.00$\pm$0.00 & 99.95$\pm$0.00 & 53.47$\pm$0.00 & 54.18$\pm$0.00 & 39.16$\pm$0.00 & 33.93$\pm$0.00\\
&& MedCLIP & 50.03$\pm$7.72 & 38.97$\pm$2.09 & 71.73$\pm$3.74 & 15.70$\pm$5.27 & 0.63$\pm$0.41 & 6.29$\pm$0.11 & 2.02$\pm$3.49 & 98.07$\pm$3.33 & 50.36$\pm$7.96 & 50.74$\pm$8.58 & 19.04$\pm$4.93 & 12.74$\pm$4.99\\
& & PubMedCLIP & 64.18$\pm$0.00 & 51.44$\pm$0.00 & 67.26$\pm$0.00 & 12.47$\pm$0.00 & 0.06$\pm$0.00 & 5.12$\pm$0.00 & 3.50$\pm$0.00 & 97.79$\pm$0.00 & 63.97$\pm$0.00 & 64.04$\pm$0.00 & 15.03$\pm$0.00 & 9.91$\pm$0.00\\

\cline{2-15}
 & \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP & 79.15$\pm$0.00 & 71.68$\pm$0.03 & 53.30$\pm$0.00 & 2.22$\pm$0.01 & 1.51$\pm$0.00 & 0.19$\pm$0.16 & 6.94$\pm$0.01 & 95.49$\pm$0.01 & 78.26$\pm$0.00 & 79.77$\pm$0.00 & 2.46$\pm$0.12 & 2.65$\pm$0.05\\
& & BLIP2 & 80.89$\pm$0.07 & 72.99$\pm$0.12 & 51.59$\pm$0.07 & 2.64$\pm$0.05 & 1.36$\pm$0.02 & 0.07$\pm$0.05 & 8.53$\pm$0.01 & 94.27$\pm$0.01 & 80.04$\pm$0.05 & 81.40$\pm$0.08 & 2.68$\pm$0.16 & 2.67$\pm$0.06\\
& & BiomedCLIP & 81.59$\pm$0.00 & 74.20$\pm$0.16 & 50.80$\pm$0.00 & 1.86$\pm$0.01 & 1.17$\pm$0.00 & 0.17$\pm$0.06 & 4.20$\pm$0.03 & 98.53$\pm$0.02 & 80.93$\pm$0.00 & 82.10$\pm$0.00 & 2.72$\pm$0.04 & 2.54$\pm$0.02\\
& & CLIP & 80.62$\pm$0.00 & 73.06$\pm$0.01 & 51.80$\pm$0.00 & 2.11$\pm$0.02 & 1.64$\pm$0.00 & 0.27$\pm$0.19 & 6.49$\pm$0.02 & 96.09$\pm$0.03 & 79.64$\pm$0.00 & 81.28$\pm$0.00 & 2.42$\pm$0.13 & 2.15$\pm$0.06\\
& & MedCLIP & 80.21$\pm$0.08 & 72.35$\pm$0.65 & 52.15$\pm$0.08 & 1.97$\pm$0.06 & 1.57$\pm$0.09 & 0.06$\pm$0.03 & 7.90$\pm$0.31 & 94.74$\pm$0.34 & 79.24$\pm$0.12 & 80.82$\pm$0.05 & 2.12$\pm$0.05 & 2.18$\pm$0.06\\
& & PubMedCLIP & 81.51$\pm$0.00 & 73.63$\pm$0.43 & 50.77$\pm$0.00 & 1.66$\pm$0.01 & 1.55$\pm$0.00 & 0.33$\pm$0.10 & 6.15$\pm$0.01 & 96.59$\pm$0.01 & 80.59$\pm$0.00 & 82.14$\pm$0.00 & 2.24$\pm$0.08 & 1.92$\pm$0.02\\
\midrule
\multirow{23}{*}{{\rotatebox{90}{PAPILA}}} & \multirow{11}{*}{{\rotatebox{90}{Linear Probe}}} & BLIP & 82.19$\pm$1.14 & 72.62$\pm$4.69 & 59.03$\pm$0.48 & 30.20$\pm$0.36 & 5.68$\pm$2.11 & 2.19$\pm$2.05 & 10.71$\pm$10.71 & 14.03$\pm$8.79 & 78.70$\pm$1.57 & 84.38$\pm$1.04 & 31.55$\pm$2.50 & 29.96$\pm$0.36\\
& & BLIP2 & 87.98$\pm$2.95 & 88.69$\pm$2.23 & 58.01$\pm$2.32 & 33.43$\pm$2.22 & 12.37$\pm$5.02 & 3.25$\pm$3.36 & 11.90$\pm$5.46 & 18.79$\pm$18.27 & 93.62$\pm$0.50 & 81.25$\pm$5.51 & 36.02$\pm$2.40 & 34.53$\pm$3.24\\
& & BiomedCLIP & 69.11$\pm$7.87 & 69.64$\pm$9.56 & 54.07$\pm$2.84 & 25.81$\pm$1.56 & 17.04$\pm$9.16 & 1.49$\pm$1.55 & 4.76$\pm$2.06 & 11.19$\pm$4.34 & 64.06$\pm$0.50 & 76.39$\pm$16.74 & 27.37$\pm$1.30 & 28.86$\pm$1.64\\
&& C2L & 67.22$\pm$3.22 & 68.45$\pm$8.91 & 69.15$\pm$1.73 & 34.09$\pm$1.21 & 15.44$\pm$13.07 & 5.68$\pm$2.02 & 7.14$\pm$7.14 & 19.23$\pm$7.55 & 65.22$\pm$6.96 & 68.23$\pm$15.89 & 34.68$\pm$3.40 & 38.10$\pm$1.95\\
& & CLIP & 82.78$\pm$9.66 & 82.74$\pm$2.23 & 65.48$\pm$0.93 & 34.19$\pm$1.84 & 4.40$\pm$1.54 & 3.95$\pm$3.75 & 14.29$\pm$12.88 & 25.07$\pm$17.66 & 84.06$\pm$11.04 & 81.42$\pm$6.47 & 38.63$\pm$1.68 & 34.69$\pm$1.41\\
& & DINOv2 & 83.06$\pm$4.88 & 80.36$\pm$6.36 & 51.29$\pm$2.39 & 25.98$\pm$1.48 & 7.25$\pm$5.76 & 2.69$\pm$2.42 & 4.76$\pm$2.06 & 15.48$\pm$13.00 & 80.00$\pm$3.98 & 86.81$\pm$7.39 & 28.64$\pm$2.09 & 26.71$\pm$1.15\\
& & MedCLIP & 78.68$\pm$1.54 & 79.76$\pm$4.69 & 62.94$\pm$0.40 & 32.61$\pm$1.25 & 8.50$\pm$8.35 & 6.39$\pm$1.10 & 8.33$\pm$5.46 & 20.04$\pm$12.70 & 72.75$\pm$2.19 & 81.25$\pm$6.51 & 31.67$\pm$1.06 & 38.06$\pm$0.24\\
&& MedLVM & 81.32$\pm$0.41 & 79.17$\pm$3.04 & 58.29$\pm$0.95 & 30.53$\pm$0.90 & 6.19$\pm$3.65 & 4.64$\pm$2.04 & 2.38$\pm$2.06 & 7.90$\pm$2.28 & 82.90$\pm$3.29 & 78.12$\pm$2.76 & 30.53$\pm$3.47 & 33.07$\pm$3.16\\
& & MedMAE & 63.28$\pm$8.36 & 54.17$\pm$12.14 & 67.32$\pm$0.33 & 32.67$\pm$0.18 & 24.23$\pm$7.72 & 2.61$\pm$2.06 & 9.52$\pm$4.12 & 17.65$\pm$3.77 & 74.93$\pm$5.08 & 50.69$\pm$12.55 & 33.21$\pm$1.80 & 35.67$\pm$1.59\\
& & MoCo-CXR & 54.65$\pm$20.94 & 53.57$\pm$29.59 & 69.03$\pm$1.08 & 35.80$\pm$0.77 & 29.04$\pm$26.66 & 3.25$\pm$2.83 & 3.57$\pm$0.00 & 15.30$\pm$4.85 & 41.45$\pm$23.66 & 70.49$\pm$23.73 & 37.07$\pm$1.87 & 40.32$\pm$0.80\\
& & PubMedCLIP & 73.05$\pm$5.50 & 75.00$\pm$9.56 & 65.18$\pm$0.30 & 33.77$\pm$2.54 & 20.66$\pm$4.96 & 2.53$\pm$1.44 & 5.95$\pm$5.46 & 11.22$\pm$6.92 & 64.06$\pm$5.51 & 84.72$\pm$5.35 & 33.56$\pm$3.00 & 35.47$\pm$1.78\\


\cline{2-15}
 & \multirow{6}{*}{{\rotatebox{90}{CLIP-ZS}}} & BLIP & 35.46$\pm$0.00 & 26.79$\pm$0.00 & 219.91$\pm$0.00 & 75.03$\pm$0.00 & 30.69$\pm$0.00 & 2.37$\pm$0.00 & 0.00$\pm$0.00 & 85.05$\pm$0.00 & 23.48$\pm$0.00 & 54.17$\pm$0.00 & 75.20$\pm$0.00 & 77.57$\pm$0.00\\
& & BLIP2 & 69.11$\pm$0.14 & 64.29$\pm$0.00 & 310.17$\pm$0.01 & 81.43$\pm$0.00 & 26.81$\pm$0.60 & 3.60$\pm$0.00 & 3.57$\pm$0.00 & 74.93$\pm$0.00 & 54.78$\pm$0.00 & 81.60$\pm$0.60 & 79.64$\pm$0.00 & 83.23$\pm$0.00\\
& & BiomedCLIP & 78.33$\pm$2.07 & 76.79$\pm$4.72 & 43.57$\pm$6.74 & 13.48$\pm$6.13 & 15.33$\pm$2.70 & 8.99$\pm$3.50 & 14.29$\pm$3.57 & 73.88$\pm$6.66 & 72.17$\pm$2.30 & 87.50$\pm$1.04 & 16.01$\pm$2.37 & 21.68$\pm$7.29\\
& & CLIP & 78.25$\pm$0.00 & 85.71$\pm$0.00 & 43.52$\pm$0.00 & 16.58$\pm$0.00 & 9.86$\pm$0.00 & 1.15$\pm$0.00 & 3.57$\pm$0.00 & 95.33$\pm$0.00 & 81.74$\pm$0.00 & 71.88$\pm$0.00 & 21.26$\pm$0.00 & 20.10$\pm$0.00\\
& & MedCLIP & 50.51$\pm$16.80 & 60.12$\pm$36.70 & 65.58$\pm$2.84 & 32.18$\pm$1.65 & 23.78$\pm$14.78 & 4.32$\pm$1.43 & 7.14$\pm$3.57 & 84.61$\pm$3.27 & 37.68$\pm$10.73 & 61.46$\pm$23.87 & 30.50$\pm$1.81 & 34.82$\pm$0.81\\
& & PubMedCLIP & 43.26$\pm$0.00 & 33.93$\pm$0.00 & 101.25$\pm$0.00 & 51.10$\pm$0.00 & 36.74$\pm$0.00 & 1.17$\pm$0.00 & 7.14$\pm$0.00 & 78.03$\pm$0.00 & 61.74$\pm$0.00 & 25.00$\pm$0.00 & 51.80$\pm$0.00 & 52.97$\pm$0.00\\
\cline{2-15}
 & \multirow{6}{*}{{\rotatebox{90}{CLIP-Adapt}}} & BLIP & 84.63$\pm$0.63 & 80.95$\pm$1.03 & 33.74$\pm$0.66 & 10.52$\pm$0.93 & 24.99$\pm$1.33 & 1.77$\pm$0.29 & 1.19$\pm$2.06 & 74.16$\pm$5.72 & 71.88$\pm$1.33 & 96.88$\pm$0.00 & 19.77$\pm$0.23 & 18.00$\pm$0.35\\
& & BLIP2 & 90.62$\pm$0.59 & 89.88$\pm$1.03 & 37.73$\pm$0.33 & 17.08$\pm$1.65 & 9.42$\pm$2.31 & 8.29$\pm$1.76 & 16.67$\pm$2.06 & 79.20$\pm$1.26 & 92.75$\pm$1.00 & 83.33$\pm$3.12 & 23.17$\pm$0.85 & 14.89$\pm$2.61\\
&& BiomedCLIP & 83.85$\pm$1.66 & 86.90$\pm$1.03 & 32.91$\pm$1.14 & 7.65$\pm$3.75 & 8.72$\pm$1.38 & 3.40$\pm$1.27 & 10.71$\pm$6.19 & 73.00$\pm$8.07 & 79.13$\pm$1.51 & 87.85$\pm$2.62 & 9.01$\pm$2.01 & 12.40$\pm$3.27\\
&& CLIP & 82.51$\pm$0.47 & 82.74$\pm$1.03 & 38.51$\pm$0.52 & 11.69$\pm$1.25 & 20.29$\pm$0.60 & 3.33$\pm$4.31 & 19.05$\pm$2.06 & 75.19$\pm$1.20 & 88.70$\pm$0.00 & 68.40$\pm$0.60 & 20.15$\pm$0.91 & 17.95$\pm$4.44\\
& & MedCLIP & 88.49$\pm$2.12 & 86.90$\pm$2.73 & 39.30$\pm$0.34 & 17.61$\pm$2.56 & 13.69$\pm$1.28 & 0.65$\pm$0.47 & 5.95$\pm$7.43 & 81.39$\pm$13.74 & 81.45$\pm$1.33 & 95.14$\pm$2.17 & 19.31$\pm$2.48 & 19.09$\pm$3.07\\
&& PubMedCLIP & 84.00$\pm$0.36 & 75.60$\pm$1.03 & 36.13$\pm$0.19 & 14.30$\pm$1.55 & 11.78$\pm$1.00 & 2.46$\pm$1.00 & 4.76$\pm$2.06 & 79.09$\pm$0.63 & 78.84$\pm$1.00 & 90.62$\pm$0.00 & 17.35$\pm$3.34 & 17.14$\pm$0.23\\


\bottomrule
\end{tabular}
\end{threeparttable}
}
% \end{sidewaystable}
\end{table}

==> sections/method_classification.tex <==

\subsection{Classification}
\label{method:cls}
% \RJ{Write a brief overview after all parts are finished.}

\subsubsection{Setup}
\textbf{Datasets}. Tab.~\ref{tab:cls_dset} details the nine datasets used for classification, including information on their modality, number of images, and sex ratio (M/F).



% \subsubsection{Foundation Models}
\textbf{Models}. 
We incorporate ten foundational models from both general computer vision and medical image analysis domains, spanning the following two main categories: 
(1) pure vision models (VMs) pre-trained using self-supervised learning (SSL) approaches; (2) vision-language models (VLMs) trained with contrastive language-image pretraining~\cite{radford2021learning}. Tab.~\ref{tab:fm_cls} lists the information of included foundation models.

\textbf{Metrics}. We present only the most insightful results/metrics in the main paper, the remaining metrics are reported in the Appendix. For \underline{\textit{(1) Utility}}, we use the \textbf{Area Under the Curve (AUC)}, which reflects the model's overall performance. For \underline{\textit{(2) Positive-Parity-Fairness}}, we report \textbf{Disparity Impact (DI)}. For \underline{\textit{(3) Outcome-Consistency-Fairness}}, we include \textbf{AUC gap ($\text{AUC}_\Delta$)}, which assesses if both groups receive approximately equal predictive performance; and \textbf{Equal Odds (EOdds)}, which measures the differences in true positive and false positive rates between advantaged and disadvantaged groups. For \underline{\textit{(4) Predictive-Alignment-Fairness}}, we report the \textbf{Expected Calibration Error Gap ($\text{ECE}_\Delta$)}, where a high value indicates an optimal decision threshold. More details and results for these criteria are explained in the Appendix. For (5) \underline{\textit{Representation fairness}}, we measure the \textbf{AUC ES} score, where a higher value stands for a better utility-fairness tradeoff.




% \textbf{Vision Models}. We consider models pretrained with popular self-supervised learning methods, including: \textbf{DINOv2}, \textbf{LVM-Med}, \textbf{MedMAE}, \textbf{MoCo-CXR}, \textbf{C2L}.  

% \textbf{Vision-Language Models}. We include \textbf{CLIP}; \textbf{BLIP2}; \textbf{MedCLIP}, \textbf{PubMedCLIP} and \textbf{BiomedCLIP}.

% Table~\ref{tab.clssFM} lists the FMs used for classification. These models include a variety of advanced encoders that's both and tailored for medical imaging tasks, highlighting their source, type, and respective links for further reference.


% \textbf{Implementation Details}. TODO


\subsubsection{Results}
\ZK{Should we merge the same conclusions for cls and seg? Such as "Trading-off utility and fairness is challenging for foundation models", "No FM significantly outperforms others in terms of utility and fairness tradeoff".}
\YZ{I'm adding a bar plot as Q1 to align with seg discussing the unfairness in FMs. So the main two questions are "Unfairness exists in foundation models", "Sex-aware utility skewness across different datasets", which are consistent for cls and seg. In cls, there is an additional section to discuss the trade-offs and compare FMs. You can decide whether to include such analysis in Seg. I think it's ok if we don't since there is already another question "Correlations between fairness, prompt types, and model dimensions" in seg.}
\ZK{Exactly, we can split the result part into the common part and the specialized part.}
\label{sec:eva_cls}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{Figs/bar_delta_auc_cls.pdf}
    \caption{Fairness of foundation models across three classification use cases (averaged over nine datasets). Error bars represent the standard deviation from three runs using different random seeds.}
    \label{fig:cls_bar}
\end{figure}

\textbf{Unfairness exists in foundation models.} Fig.~\ref{fig:cls_tradeoff} presents utility-fairness trade-off results of three downstream classification use cases supported in \ours. All models exhibit biased performance between males and females across various fairness metrics, compromising the utility-fairness trade-off. Generalized vision-language models show poor zero-shot performance in terms of both utility and fairness. However, simple adaptations significantly enhance the utility-fairness trade-off.

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{Figs/scatter_cls.pdf}
    \caption{Fairness-utility trade-off on classification tasks (average across all nine datasets).}
    \label{fig:cls_tradeoff}
\end{figure}

% \subsubsection{Bias Mitigation Strategies}


% \subsubsection{Bias widely exists among different medical datasets and FMs}
% % scatter plot
% % t-SNE (optional)

% \subsubsection{Finetune balances the utility and fairness tradeoff}
% % scatter plot

\textbf{No FM significantly outperforms others in terms of utility and fairness tradeoff}. 
% \YZ{@Ruinan, Zikang is using ES-Dice, which is a single metric to represent utility/fairness trade-offs. Therefore, I added a new evaluation aspect in Sec. 2.4, which is not yet covered in the evaluation of classification. However, I think it might be appropriate if we use a ES-AUC metric (which is simple to calculate based on overall auc and subgroup auc) here, since we are comparing tradeoffs here. And ES-AUC will be a metric that directly represents such trade-offs which fits these comparisons. In this case, we can use CD diagrams of (1) overall AUC, (2) delta AUC, (3) ES-AUC. What do you think? ES-AUC calculation reference: https://arxiv.org/pdf/2306.09264. Also can align with the calculation of ES-Dice used by Zikang.}\RJ{Good idea. Will edit CD figures.
% }


% AUC, delta_AUC, ES_AUC
\begin{figure}[H]
    \centering
    \begin{minipage}[b]{\textwidth}
        \centering
        \includegraphics[width=0.32\textwidth]{Figs/cd_cls/lp/Overall AUC.pdf}
        \includegraphics[width=0.32\linewidth]{Figs/cd_cls/lp/AUC Gap.pdf}
        \includegraphics[width=0.32\textwidth]{Figs/cd_cls/lp/AUC ES.pdf}
        \caption{Linear Probing: Overall AUC, AUC GAP, AUC ES.}
        \label{fig:}
    \end{minipage}\\
    % \hfill
    \begin{minipage}[b]{\textwidth}
        \centering
        \includegraphics[width=0.32\textwidth]{Figs/cd_cls/clipadapt/Overall AUC.pdf}
        \includegraphics[width=0.32\linewidth]{Figs/cd_cls/clipadapt/AUC Gap.pdf}
        \includegraphics[width=0.32\textwidth]{Figs/cd_cls/clipadapt/AUC ES.pdf}
        \caption{CLIP-Adaptor: Overall AUC, AUC GAP, AUC ES.}
        \label{fig:}
    \end{minipage}\\
\end{figure}

\textbf{Sex-aware utility skewness across different datasets}. Among the datasets we used, there is 

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{Figs/scatter_cls/scatter_cls.pdf}
\end{figure}

% \subsubsection{Fairness among datasets and geners}

% \subsubsection{TODO: Fairness in PEFT}




















==> sections/method_segmentation.tex <==
\subsection{Segmentation}\label{method:seg}

    
\subsubsection{Setup}

\paragraph{Datasets.}
Four 2D datasets and Four 3D datasets are selected for evaluating the fairness of the segmentation models. These datasets vary in modality (dermatology, ultrasound, OCT, X-ray, CT, and MRI), body parts (brain, eyes, skin, thyroid, chest, liver, kidney, and spine), and the number of masks (ranging from two to more than six). The details of the datasets are shown in Tab.~\ref{tab.SegDatasets}.

\paragraph{Models.}
Among the SAM-family models, we select 9 models from three categories. i.e. SAM models trained with natural images (SAM~\citep{kirillov2023segment}, MobileSAM~\citep{zhang2023faster}, and TinySAM~\citep{shu2023tinysam}), SAM models that takes 2D images as input (MedSAM~\citep{ma2024segment}, SAM-Med2D~\citep{cheng2023sammed2d}, and FT-SAM~\citep{cheng2023sammed2d}), and SAM models that directly process 3D volumes (SAM-Med3D~\citep{wang2023sam}, FastSAM3D~\citep{shen2024fastsam3d}). We also include SegVol~\citep{du2023segvol}, which is an interactive 3D image segmentation model that can accept points and bounding box prompts. 
The details of the 9 models can be found in Tab.~\ref{tab.SegModels}.

\paragraph{Metrics.}
We present only the most insightful results/metrics in the main paper, the remaining metrics are reported in the App.
For \underline{\textit{(1) Utility}}, we use the \textbf{Dice Similarity Score (DSC)}, which reflects the model's overall performance. 
% For \underline{\textit{(2) Positive-Parity-Fairness}}, we report \textbf{Disparity Impact (DI)}. 
For \underline{\textit{(2) Outcome-Consistency-Fairness}}, we include \textbf{DSC gap ($\text{DSC}_\Delta$)} and \textbf{DSC standard deviation ($\text{DSC}_{\text{STD}}$)}, which assesses if both groups receive approximately equal predictive performance; 
besides, we also include \textbf{DSC skewness ($\text{DSC}_{\text{Skew}}$)}, which measures the degree of skewness of DSC between advantaged and disadvantaged groups.
For \underline{\textit{(3) Utility-Fairness-tradeoff}}, we report the \textbf{Equity-Scaled DSC ($\text{DSC}_\text{ES}$)}, which measures the tradeoff between overall utility and utility variations. 
More details and results for these criteria are explained in the App.
\ZK{Move $DSC_{\text{STD}}$ to App., as we only consider binary attributes. Here the 3 points are not totally aligned with classification, is it OK?} 
\YZ{Yuan: I think we need to align with the evaluation aspects in Sec.~\ref{sec:pipline_metric}? The first two categories here seem great. Can $DSC_{ES}$ be categorized as Predictive-Alignment-Fairness in Sec.~\ref{sec:pipline_metric} according to definition? If not, we can compromise and make up another definition that works for all of us.}
\ZK{Predictive-Alignment-Fairness mainly focuses on the calibration, $DSC_{ES}$ is about the trade-off between utility and fairness. Is it able to add a new category `Utility-Fairness-Trade-off'? Perhaps $\frac{AUC_{Avg}}{1 + AUC_{STD}}$?}\RJ{Good idea to add a new category of metrics, adds an additional point to our contribution. From my writing today, I have the feeling that we don't need every metrics/visualization in every point, but it's important that we at least include one point in Tab.~\ref{tab:baseline_benckmark}, where we declare our contribution there. Others can go to App.}








\subsubsection{Results}
\paragraph{Unfairness exists in various medical datasets.}
Firstly, we directly evaluate six 2D-SAMs and three 3D-SAMs on the four 2D and four 3D datasets. For each dataset and model, we select the prompt with the highest overall utility and calculate the delta DSC. The results are shown in Fig.~\ref{fig.SegOverall}. From the figure we can find that unfairness exists in various medical datasets, and the degree of unfairness varies across different datasets. For example, SegVol shows a disparity of more than $10 \%$ on the IRCADb dataset, which is unacceptable in medical applications.
This finding have been discovered and reported in previous works but has not been systematically studied in FM-based segmentation models. This unfair situations also exist in other attributes inlcuding age, race, etc. (see App.~\ref{}).

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{Figs/DSC_overall.pdf}
    \caption{Unfairness exists in various medical datasets}\label{fig.SegOverall}
    % \label{fig:enter-label}
\end{figure}

\paragraph{Sex-aware utility skewness is consistent within dataset.}
We further investigate the utilities skewness between the Male and the Female. As shown in Fig.~\ref{fig.stats}, the utility skewness is basically consistent within each dataset, despite of the type of SegFMs. For example, SegFMs perform worse on the Male group than the Female group in the HAM10000 dataset, while it is easier for SegFMs to segment lung for the Male group in the Montgomery dataset.
Besides, compared to 3D models, this trend is more consistent for 2D models. Potential reasons for this phenomenon could be the differences in the size of the masks (the mask in 3D datsets are larger) and the number of classes of masks (3D datasets have more than 2 classes of masks). This task complexity may lead to the performance variations for different SegFMs.

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{Figs/F-M.pdf}
    \caption{Sex-aware utility skewness is consistent within dataset.\textcolor{#FFBE7A}{$\bullet$}:General purpose SegFMs}\label{fig.stats}
    % \label{fig:enter-label}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{minipage}[b]{\textwidth}
        \centering
        \includegraphics[width=0.32\textwidth]{Figs/cd_seg/Rank_Avg.pdf}
        \includegraphics[width=0.32\linewidth]{Figs/cd_seg/Rank_absDelta.pdf}
        \includegraphics[width=0.32\textwidth]{Figs/cd_seg/Rank_ES.pdf}
        \caption{2D SegFMs: $\text{DSC}_{\text{Avg}}, \text{DSC}_{\Delta}, \text{DSC}_{\text{ES}}$.\ZK{A problem: these 6 models result in 3 groups in CD if measured on both 2D and 3D datsets. If we only evaluate on 2D datasets, the conclusion is consistent with CLS.}}
        \label{fig:}
    \end{minipage}
\end{figure}

% \paragraph{Corrlations between fairness, prompt types, and model dimensions.}
\paragraph{Careful selection of FMs is needed for ensuring fairenss.}
Further, we evaluate whether the selection of elements in FMs affects fairness of the outcome.
Here, we consider two main components of SegFMs, i.e. the choice of prompts (including \emph{center}, \emph{rand}, \emph{rands}, and \emph{bbox}), and the types of SegFMs (including 2D General-SegFMs, 2D Med-SegFMs, and 3D Med-SegFMs).
For the \textbf{choice of prompts}, we average the $\text{DSC}_\Delta$ ratio of SAM-Med2D on all the eight datasets, which is defined as ${\text{DSC}_\Delta} / {\text{DSC}}$.
As shown in Fig.~\ref{fig.element}~(a), compared to \emph{center} and \emph{rand}, models using \emph{rands} and \emph{bbox} tends to be more unfair across different datasets. This might due to the tighter constraints on the segmentation which provided by \emph{rands} and \emph{bbox}.
For the \textbf{type of SegFMs}, we average the $\text{DSC}_\Delta$ ratio across the eight datasets following the taxonomy introduced in Sec.~\ref{sec.benchmarkSeg}. Surperisingly, the 2D General SegFMs is the fairest among the three categories, followed by 2D Med-SegFMs, while 3D Med-SegFMs have the worst fairness.
These findings suggest that careful selection of FMs is needed to ensure fairness in healthcare applications. 


\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{Figs/elements.pdf}
    \caption{(a) Compared to \emph{center} and \emph{rand}, using \emph{rands} and \emph{bbox} prompts tends to have lower $\text{DSC}_{\Delta}$ ratio (using SAMMed2D as an example). (b) }\label{fig.element}
\end{figure}




\paragraph{Existing unfairness mitigation strategies are not always effective.}
Lots of unfairness mitigation methods for traditional neural networks have been proposed in the literature. However, the effectiveness of these methods on FMs is still unknown.
Here, we examine three mitigation algorithms for classification and segmentation, respectively.
For classification, we apply these methods on \ZK{xxx dataset} by fine-tuning the LP and LoRA part, while experiments for segmentation are conducted on the HAM10000 dataset following the SAMed pipeline in~\citep{samed}.



% \begin{table}[htbp]
%     \caption{Evaluation of Unfairness Mitigation Methods. \best{Best} and \secb{second best} results are highlighted.}\label{tab.SegMitigation}
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lcccccccc}
%     \toprule
%     {\textbf{Method}} & $\text{DSC}_{\text{Avg}}\uparrow$ & $\text{DSC}_{\text{Female}}$ & $\text{DSC}_{\text{Male}}$ &  $\text{DSC}_{\Delta}\downarrow$ & $\text{DSC}_{\text{STD}}\downarrow$ & $\text{DSC}_{\text{Skew}}\downarrow$ & $\text{DSC}_{\text{ES}}\uparrow$\\
%     \midrule
%     SAM (best) & 83.55 & 84.47 & 82.74  & 1.73 & 0.86  & 1.11 & 82.83 \\ 
%     \midrule
%     SAMed &  90.92 & 90.98 & 90.87  & \secb{0.10} & \secb{0.05}  & \secb{1.01} & 90.87 \\
%     SAMed + FEBS & \best{91.63} & \best{91.64} & \best{91.62}  & \best{0.02} & \best{0.01}  & \best{1.00} & \best{91.62} \\
%     SAMed + Resampling & \secb{91.51} & \secb{91.60} & \secb{91.43}  & 0.17 & 0.09  & 1.02 & \secb{91.43} \\
%     SAMed + InD  & 88.85 & 89.61 & 88.19  & 1.42 & 0.71  & 1.14 & 88.22 \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{table}
% The fairness-utility plot is shown in Fig.~\ref{fig.mitigation}. Following~\citep{fairadabn}, we split the space into four quadrants. Among the three methods, only SAM + FEBS achieves both better utility and fairness (top left quadrant), while SAM + InD results in the worst fairness and utility (bottom right quadrant). This indicates that unfairness mitigation methods are not always effective for SegFMs.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{Figs/tradeoff.pdf}
%     \caption{Unfairness mitigation methods are not always effective. Top left: High utility, High fairness; Top right: High utility, Low fairness; Bottom left: Low utility, High fairness; Bottom right: Low utility, Low fairness.\ZK{Perhaps draw a line with the same ES? By using $\Delta$ to represent $STD$}}\label{fig.mitigation}
% \end{figure}

\newpage



% \begin{figure}
%     \centering
%     \includegraphics[width=0.6\textwidth]{Figs/scatter_debias.pdf}
%     \caption{Fairness-utility trade-off of bias mitigation fine-tuning methods (average across 3 datasets).}
% \end{figure}


% \subsubsection{Unfairness Mitigation}




==> sections/relatedwork.tex <==
\section{Related Work}

\noindent\textbf{Fairness in medical image analysis.}
While most of the research in deep-learning-based medical image analysis focuses on improving model utility in various downstream tasks, some researchers witnessed a serious and widespread issue, i.e. these algorithms tend to perform unfairly towards marginalized populations. 
For example, Seyyed-Kalantari~\textit{et al.}~\citep{seyyed2021underdiagnosis} find that their Chest X-ray classifier has a higher underdiagnosis rate for Hispanic female patients.
Similar phenomenons also occur in other medical tasks, including regression~\citep{piccarra2023analysing}, segmentation~\citep{puyol2021fairness}, reconstruction~\citep{du2023unveiling}, etc. 
This fairness issue must be taken into consideration as it not only guarantees health equity for patients with different demographics but improves the model's transparency, interpretability, and trustworthiness, which provides confidence for adopting them in clinical applications.

% 4. Recent progress in solving fairness in FMs

\noindent\textbf{Foundation models in medical image analysis.}
FMs, which are usually trained on numerous datasets, show powerful zero-shot utilities on various downstream tasks.
Recently, researchers have adopted this new generation of deep learning models for medical image analysis, especially in classification and segmentation.
Classificaiton FMs vary in architecture, i.e., some FMs only take images as input, trying to learn a general representation across diverse datasets by SSL (such as MedMAE~\citep{xiao2023delving} and MedLVM~\citep{nguyen2023lvm}), while the other FMs extract features via language-image alignment (such as MedCLIP~\citep{wang2022medclip}, PubMedCLIP~\citep{eslami2021does}).
As for segmentation FMs, after the advent of SAM~\citep{kirillov2023segment}, there are a series of works that propose to use FMs for medical image segmentation, including MedSAM~\citep{ma2024segment}, Slide-SAM~\citep{quan2024slide}, etc.
However, most of these works focus on improving the model's utility, while fairness is often overlooked.


% \noindent\textbf{Medical Segmentation FMs.}




==> sections/results.tex <==
% \section{Results \& Discussion}


